Seeing or Guessing? An Empirical Study of Spatial Bias in Vision-Language Models via Counterfactuals

Spatial intelligence is essential for embodied tasks such as navigation, manipulation, and agentic interaction. Vision-Language Models (VLMs) increasingly exhibit spatial reasoning capabilities, yet priors learned from large-scale vision-language pre-training may override current visual evidence and induce systematic spatial errors. While social bias and visual hallucination have been widely studied, spatial bias remains underexplored. We define spatial bias as the systematic tendency of VLMs toward prior-aligned spatial predictions despite conflicting visual evidence. To investigate this phenomenon, we construct SpatialCF-Bench, a paired counterfactual embodied visual question answering (VQA) benchmark spanning diverse spatial tasks and bias priors, and introduce a multi-stage diagnostic framework that distinguishes counterfactual failures from prior-retention bias, language-aligned bias, and non-bias errors. We further investigate how input organization, contrastive context, background information, and visual guidance affect spatial bias, and evaluate multiple mitigation strategies. Experiments on diverse VLMs reveal widespread spatial bias that varies across model family, spatial task, prior source, and contextual conditions such as memory and visual information. Input and background configurations affect counterfactual robustness, while selective context suppression and explicit visual guidance can reduce bias. Prompt-based interventions yield limited and inconsistent gains, whereas supervised fine-tuning provides more reliable mitigation. These findings underscore the limitations of accuracy-only evaluation and the need to explicitly diagnose and mitigate spatial bias in embodied VLMs.

==> sections/Benchmark.tex <==
\section{Spatial Bias Benchmark}

\textbf{Overview.}
We introduce a paired original--counterfactual VQA dataset for diagnosing spatial bias in embodied aerial imagery.
Each pair shares the same question and four answer choices but contains an original image and a counterfactual counterpart with image-specific ground-truth answers.
The dataset covers six spatial tasks and four bias-source categories defined in Sec.~\ref{sec:spatial_bias} and Fig.~\ref{fig:bias_type}.
By keeping the linguistic input fixed while modifying task-relevant visual evidence, this design enables controlled evaluation of counterfactual spatial reasoning.

\textbf{Dataset Statistics.}
The dataset contains 1,254 original--counterfactual pairs (2,508 images) spanning all 24 task--source combinations.
As shown in Fig.~\ref{fig:data}, the data are relatively balanced across spatial tasks, bias sources, and answer positions.
Detailed statistics and representative examples are provided in Appendix~\ref{app:benchmark}.

\begin{figure}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/data.pdf}
    \caption{\textbf{Distribution of spatial tasks and bias sources.}
    Left: Distributions across four bias sources (inner ring) and six spatial tasks (outer ring).
    Right: Joint distribution over the 24 task--source combinations.}
    \label{fig:data}
    \vspace{-5pt}
\end{figure}

\textbf{Construction Pipeline.}
We construct the dataset from multi-source real-world aerial imagery \cite{du2019visdrone,liu2023robust,nie2025m3ot,du2018uavbenchmark} following the six-task, four-source taxonomy in Fig.~\ref{fig:bias_type}.
For each original image, we create a counterfactual counterpart through targeted visual editing while preserving the question and answer choices, and annotate image-specific ground-truth answers.
We then perform visual-quality inspection, task-consistency verification, label normalization, duplicate removal, and model-assisted validation to filter invalid samples, resulting in the final 1,254 pairs.
Further construction and validation details are provided in Appendix~\ref{app:data_cons}.

% \textbf{Overview.}
% We introduce a paired original-counterfactual VQA dataset for diagnosing spatial bias in embodied aerial imagery. Each sample contains an original image and a counterfactual counterpart, paired with the same question and four answer choices but independently annotated ground-truth answers. The dataset covers six spatial tasks and four bias-source categories, as introduced in Sec.~\ref{sec:spatial_bias} and Fig.~\ref{fig:bias_type}. By holding the linguistic input fixed while modifying task-relevant visual evidence, the paired design enables controlled analysis of counterfactual spatial reasoning.

% \textbf{Dataset Statistics.}
% The dataset contains 1,254 original--counterfactual pairs (2,508 images) spanning all $6\times4=24$ task--source combinations. Each spatial-task category contains 187--234 pairs (14.9\%--18.7\%), while each bias-source category contains 306--331 pairs (24.4\%--26.4\%); individual combinations contain 38--65 pairs. As shown in Fig.~\ref{fig:data}, the dataset is relatively balanced across both dimensions. The four answer positions are also approximately balanced for both original and counterfactual samples. Please refer to Appendix~\ref{app:benchmark} for more information of dataset statistics and representative examples.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figs/data.pdf}
%     \caption{\textbf{Distribution of spatial tasks and bias sources.} Left: Distributions of 4 bias sources (inner ring) and 6 spatial tasks (outer ring). Right: Joint distribution of 24 task--source combinations.
%     }
%     \label{fig:data}
%     \vspace{-5pt}
% \end{figure}

% \textbf{Construction Pipeline.}
% We construct the dataset from multi-source aerial imagery following the six-task, four-source taxonomy in Fig.~\ref{fig:bias_type}. For each original image, we create a counterfactual counterpart through targeted visual editing while preserving the question and answer choices, and annotate image-specific ground-truth answers. After visual-quality checks, task-boundary verification, label normalization, and duplicate removal, we obtain 1,297 candidate pairs. We further evaluate the candidates using Doubao Seed 2.1 Pro, MiniMax M3, and Qwen3-VL Plus to remove invalid pairs for which all four models fail on the original image. More dataset construction details can be found in Appendix \ref{app:data_cons}.

% \textbf{Overview.}
% % probing design: counterfactual image edition
% We introduce a paired visual question answering dataset for investigating spatial reasoning biases in aerial imagery. Each sample consists of an original image and a counterfactual counterpart, evaluated using the same question and four answer options, with separately annotated answers. The dataset spans six spatial tasks and four bias-reason categories: cultural and behavioral norms, reference-frame transformations, physical–geometric principles, and semantic co-occurrence. This paired design enables comparisons of model responses to controlled visual changes while holding the linguistic input fixed.

% \textbf{Dataset Statistics.}
% The dataset contains 1,254 image pairs, comprising 2,508 images, and covers all 24 combinations of spatial tasks and bias reasons. Spatial-task categories contain 187–234 pairs each, accounting for 14.9\%–18.7\% of the dataset, while bias-reason categories contain 306–331 pairs each, accounting for 24.4\%–26.4\%. Individual task–reason combinations contain 38–65 pairs. As illustrated in Fig.\ref{fig:data}, the dataset provides relatively balanced coverage of both classification dimensions. Ground-truth answer positions are also approximately balanced across the four options for both original and counterfactual images.
% \begin{figure}
%     \centering
%     \includegraphics[width=0.95\linewidth]{figs/data.pdf}
%     \caption{\textbf{Distribution of spatial tasks and bias reasons in the dataset.} Left: the inner pie shows the four bias-reason categories, while the outer ring shows the six spatial-task categories; the two layers represent separate marginal distributions. Right: the Sankey diagram depicts the joint distribution of the 24 tasks, with ribbon widths proportional to the number of sample pairs in each task–reason combination. 
%     Counts and percentages are computed over all original–counterfactual pairs.
%     }
%     \label{fig:data}
% \end{figure}

% \textbf{Construction Pipeline.}
% We construct a total of original-counterfactual data samples with $6\times4=24$ categories covering various spatial reasoning tasks and potential bias sources shown in Fig.\ref{fig:bias_type}.
% Dataset construction begins with multi-source aerial imagery and a taxonomy of six spatial tasks and four bias reasons. Counterfactual counterparts are constructed through targeted visual edits, accompanied by shared multiple-choice questions and image-specific answer annotations. Following recorded visual and task-boundary checks, label normalization, and duplicate handling, 1,297 candidate pairs are assembled. We then evaluate these pairs using Doubao Seed 2.1 Pro, MiniMax M3, Qwen3-VL Plus, and Qwen3-VL-8B. A model-based filtering rule excludes pairs for which all four models answer the original image incorrectly but the counterfactual image correctly. This removes 43 pairs (3.32\%), yielding the final dataset of 1,254 pairs.

% \subsection{Task Setup}


==> sections/Bias_mitigation.tex <==
\section{Bias Mitigation}
\label{sec:bias_mitigation}

This section investigates four representative strategies for mitigating spatial bias, covering both inference-time intervention and parameter-level adaptation: zero-shot linguistic intervention, chain-of-thought (CoT) prompting, few-shot prompting, and supervised fine-tuning (SFT). The first three methods modify model behavior without updating parameters, while SFT explicitly adapts the model using paired counterfactual supervision. Complete prompts for CoT and few-shot schemes and training configurations are provided in Appendix~\ref{app:bias_mit}.

\textbf{Zero-shot Linguistic Intervention.}
We explicitly instruct the model to prioritize current visual evidence over learned priors.
This intervention tests whether spatial bias can be reduced through lightweight instruction-level guidance without modifying the model or providing demonstrations. The added linguistic prompt \cite{sun2026vlms} follows: 
\begin{tcolorbox}[
    colback=gray!8,
    colframe=black!60,
    boxrule=0.4pt,
    arc=2pt,
    left=8pt,right=8pt,top=4pt,bottom=4pt
]
Base your judgment solely on direct visual evidence in the provided image.
Do not use your prior knowledge to choose the answer.
\end{tcolorbox}

\textbf{CoT Incorporation.}
We introduce structured reasoning that requires the model to first identify the relevant visual targets and reference frame, then infer the spatial relation, and finally verify the selected answer against visible evidence.
The goal is to reduce shortcut reasoning by encouraging explicit visual grounding before prediction.

\textbf{Few-shot Prompting.}
We provide three original--counterfactual demonstrations before inference, where the question and options remain unchanged but the correct answer may change with the visual evidence.
These examples explicitly illustrate the desired counterfactual behavior and test whether bias-aware reasoning can be induced through in-context learning.

\textbf{SFT with LoRA.}
We further perform supervised fine-tuning (SFT) on paired original and counterfactual samples to directly associate visual changes with corresponding answer changes.
The dataset is split into training, validation, and test sets at approximately $7{:}1{:}2$.
Each original--counterfactual pair contributes two independently supervised VQA examples, enabling the model to learn that identical linguistic inputs may require different predictions when the visual evidence changes.
We adopt LoRA-based parameter-efficient fine-tuning \cite{hu2022lora} and evaluate the adapted models on the same held-out test set as the prompting-based methods.
Detailed optimization settings are provided in Appendix~\ref{app:bias_mit}.



% \section{Bias Mitigation}
% \label{sec:bias_mitigation}
% In this section, we try different methods to mitigate the spatial bias in VLMs. Specifically, The detailed and complete bias mitigation prompts are provided in Appendix \ref{app:bias_mit}.
% \\
% % how to reduce spatial bias
% \textbf{Zero-shot Linguistic Intervention.} We add two sentences in the prompt for model evaluation as follows to require the system avoid the dependency on prior knowledge and pay more attention to the actual input.
% \begin{tcolorbox}[
%     colback=gray!8,
%     colframe=black!60,
%     boxrule=0.4pt,
%     arc=2pt,
%     left=8pt,right=8pt,top=4pt,bottom=4pt
% ]
% Base your judgment solely on direct visual evidence in the provided image.
% Do not use your prior knowledge to choose the answer.
% \end{tcolorbox}

% \textbf{CoT Incorporation.}
% We add multi-step thinking requirements to push the model to rethink their answers and focus more on the visual evidence by invoking their step-by-step thinking abilities. Specifically, the CoT intervention prompt follows:
% \begin{tcolorbox}[
%     colback=gray!8,
%     colframe=black!60,
%     boxrule=0.4pt,
%     arc=2pt,
%     left=8pt,right=8pt,top=4pt,bottom=4pt
% ]
% Work through the visual task step by step before choosing the final option:\\
% 1. Locate the exact target object(s) in the TARGET image, using the question's
%    descriptors. State only visible identifying cues; do not invent hidden details.\\
% 2. Specify the reference frame and decision rule in the question. Keep image-plane
%    position/projected size distinct from scene depth/physical size and object-centered
%    orientation. Describe the visible relation or property that answers this question. \\
% 3. Compare that observation with the options. Check the best competing option for
%    a visible contradiction. Prefer what is depicted over what is normally expected.
%    Select an insufficient-visibility option only if the target evidence supports it.
% \\
% Output four lines. Keep each of the first three lines to one short sentence and
% keep the total explanation under 100 words. Do not mention an answer letter until
% the final line. Use this format:
% \\
% TARGET: \textless visible target identification\textgreater \\
% EVIDENCE: \textless reference frame and observed spatial evidence\textgreater \\
% CHECK: \textless brief option comparison grounded in that evidence\textgreater \\
% ANSWER=\textless one uppercase letter A, B, C, or D\textgreater \\
% The final line must be the only ANSWER= marker. Do not output any text after it.
% \end{tcolorbox}

% \textbf{Few-shot prompting.}
% We feed the model three representative examples before test to tell the model that the input images are different and the answers might be flipped to steer the model toward visual evidence instead of prior knowledge.
% \begin{tcolorbox}[
%     colback=gray!8,
%     colframe=black!60,
%     boxrule=0.4pt,
%     arc=2pt,
%     left=8pt,right=8pt,top=4pt,bottom=4pt
% ]
% You will first see three worked examples. Each example contains an ORIGINAL image
% and a COUNTERFACTUAL (CF) image, the same question and options, and the correct
% option for each image. The examples show that changing visible evidence can
% change the correct answer even when the question and options stay the same.
% Learn to judge the image actually supplied, rather than repeating an earlier
% answer or choosing what would normally be expected. A new answer is allowed to
% change, but do not force a change merely because an image looks unusual.
% The examples are independent scenes. Their answer letters are not a pattern
% to copy. After the examples, answer only the TARGET question using the TARGET
% image. Never transfer an object or a spatial fact from an example to the target.

% EXAMPLE 1 — ORIGINAL image: ...
% \\
% EXAMPLE 1 — CF image: ...
% \\
% EXAMPLE 1 question (applies to both images): ...
% \\
% EXAMPLE 1 options:
% A. ...
% B. ...
% C. ...
% D. ...
% \\
% Correct option for ORIGINAL: ...
% \\
% Correct option for CF: ...
% \\
% The same question has different correct options because the visible evidence changed.
% \\
% END OF EXAMPLE 1.

% EXAMPLE 2 ...

% EXAMPLE 3 ...

% \end{tcolorbox}


% \textbf{SFT on original--counterfactual pairs.}
% We investigate whether supervised exposure to original and counterfactual examples can mitigate spatial bias. We partition the dataset into training, validation, and test sets at an approximately 7:1:2 ratio, comprising 877, 126, and 251 image pairs, respectively. Each original--counterfactual pair is assigned to the same split. Samples linked by identical image hashes, shared source images, or identifiable video sequences are also grouped within a single split to reduce source overlap. All three models use the same partition.

% Each training pair contributes two separate image--question--answer examples, yielding 1,754 training examples. The original and counterfactual images are presented independently with the same question and answer options, each supervised using its corresponding ground-truth answer. This exposes the model to changes in visual evidence and their associated answer changes. We minimize the autoregressive cross-entropy loss over the assistant response, formatted as \texttt{ANSWER=<letter>}, and its termination token; prompt and image tokens are excluded from the loss. Text-only inputs and reasoning traces are not included in training.

% We perform parameter-efficient fine-tuning with LoRA, using a rank of 16, a scaling factor of 32, and a dropout rate of 0.05. Adapters are applied to the attention and feed-forward projections of the language decoder, while all original model parameters remain frozen. We train for three epochs using AdamW with a learning rate of $5\times10^{-5}$, weight decay of 0.01, an effective batch size of 16, and a cosine learning-rate schedule with 17 warmup steps. For each model, we select the epoch checkpoint with the lowest validation response-token cross-entropy. At test time, we retain the corresponding P0 prompt and image preprocessing, and evaluate all mitigation methods on the same held-out test set.



==> sections/Bias_probe.tex <==
\section{Bias Diagnostic Framework}
\label{bias_diag}
% where does spatial bias emerge?

\subsection{Multi-stage Bias Diagnostic Pipeline}

To distinguish spatial bias from generic spatial errors and further identify its association with language priors, we introduce a three-stage diagnostic pipeline, as illustrated in Fig.~\ref{bias_diag}.

\begin{itemize}[nosep,leftmargin=*]
    \item \textbf{Stage 1: Baseline Sanity Test.}
    We first evaluate each VLM on the original VQA pair. Only samples correctly answered on the original input are retained for subsequent diagnosis, ensuring that failures on counterfactual inputs are not simply caused by insufficient baseline spatial capability.

    \item \textbf{Stage 2: Counterfactual Bias Test.}
    We then replace the original image with its counterfactual counterpart while keeping the question and answer options unchanged. A correct counterfactual prediction indicates successful adaptation to the modified spatial evidence. Otherwise, the sample is treated as a counterfactual failure. In particular, if the model retains the original ground-truth answer despite a changed counterfactual ground truth, we identify an \emph{original-prior retention bias}; other incorrect predictions are passed to the next stage for further attribution.

    \item \textbf{Stage 3: Text-only Blind Test.}
    Finally, we remove the image and query the model using text alone to assess language-prior dependence. If an incorrect counterfactual prediction matches the text-only prediction, we identify a \emph{language-aligned bias}. If an original-prior retention error is not aligned with the text-only prediction, it is categorized as \emph{non-language-aligned bias}. Counterfactual errors matching neither the original prior nor the text-only prediction are treated as \emph{non-bias spatial errors}.
\end{itemize}

This pipeline separates baseline capability, counterfactual failure, prior-retention bias, language-aligned bias, and residual non-bias errors in a unified manner. For finer-grained diagnosis, we further provide a hierarchical framework that localizes failures to the visual, multimodal interaction, and decision layers of VLM inference. Details are provided in Appendix~\ref{app:diag_frame}.

% \subsection{Multi-stage Language-prior Bias Diagnostic Pipeline}
% To investigate a more fine-grained spatial bias and error occurrence positioning, as well as the attribution of them during the model reference process,  
% % and what is the main cause of the bias, 
% we propose a three-stage spatial bias diagnostic framework, as illustrated in Fig. \ref{bias_diag}.
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Stage 1: Baseline Sanity Test.} At the very first stage, we take the input as both spatial-related query text and original ordinary images to verify that the subjects in the dataset are known to VLMs. Only if VLMs succeed to do the spatial reasoning in these unaltered raw data, can we take it as a vlid sample and attribute their failures on the edited counterfactual images to potential language bias later.
    
%     \item \textbf{Stage 2: Counterfactual Bias Test.} At this stage, we use the built counterfactual image shared the same question and options with the original pair to dig out the bias of the model. If the model select the answer identical to the baseline sanity test under the condition that the GT answers are different from the original samples and its corresponding counterfactual counterparts, it can be seen as influenced by the original vision-language pair priors. Otherwise, the errors can be caused by other spatial reasons such as visual feature collapse, multimodal misalignment, and reasoning errors.
    
%     \item \textbf{Stage 3: Text-only Blind Test.} 
%     At this stage, we further classify the spatial bias and error into non-bias spatial error, language-prior bias, or non-language-prior bias by conducting text-only blind test without image input. For the spatial error categorized from the previous stage, if the text-only prediction equals counterfactual prediction, there exists a language-prior bias since text overrides, else if not, a non-bias spatial error exists. For the spatial bias category, if the text-only prediction is identical to the original GT answer, there is also a language-prior bias as the sample is highly language-dependent. But if not, the bias is non-language-prior.
% \end{itemize}
% For further diagnosis of spatial errors caused by visual feature collapse, multi-modal misalignment, reasoning errors, and prior bias, we also provide a more fine-grained multi-stage hierarchical diagnostic framework by locating the errors in the visual layer, interaction layer, and decision layer during the model inference, as illustrated in Appendix \ref{app:diag_frame}.

% We mainly categorize the diagnostic results into the following 3 main branches covering 6 diagnostic types: 
% \begin{itemize}[leftmargin=*]
%     \item[(a] No Spatial Error:
%     \begin{itemize}
%         \item No Spatial Bias:
%         \item Beneficial Spatial Bias:
%     \end{itemize}
%     \item[(b] Spatial Bias:
%     \begin{itemize}
%         \item Language-prior Bias:
%         \item Non-Language-prior Bias:
%     \end{itemize}
%     \item[(c] Spatial Error: 
%     \begin{itemize}
%         \item Bias-caused Spatial Error:
%         \item Non-bias Spatial Error:
        
%     \end{itemize}
% \end{itemize}


\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figs/bias_diag.pdf}
    \caption{\textbf{Multi-stage spatial bias diagnostic framework.} Baseline sanity, counterfactual bias, and text-only blind tests.
    }
    \label{fig:bias_diag}
\end{figure}

\subsection{Metrics Beyond Accuracy}

Accuracy alone cannot reveal whether spatial failures are random or systematically associated with learned priors.
We therefore introduce a set of diagnostic metrics to characterize spatial capability, counterfactual failure, bias prevalence, and language-prior dependence through the following research questions (RQs):

\begin{itemize}[nosep,leftmargin=*]
    \item[] \textbf{RQ1: Spatial Reasoning Performance.}
    How well do VLMs maintain accurate and consistent spatial reasoning across original and counterfactual conditions?

    \item[] \textbf{RQ2: Counterfactual Failure.}
    What proportion of counterfactual failures are attributable to bias-related versus non-bias errors?

    \item[] \textbf{RQ3: Spatial Bias Prevalence.}
    To what extent do VLMs retain or follow prior-consistent spatial predictions despite contradictory counterfactual evidence?

    \item[] \textbf{RQ4: Language-prior Prevalence.}
     What fraction of eligible samples exhibit a language prior toward the original spatial answer without visual evidence?

    \item[] \textbf{RQ5: Language-prior Dominance.}
    When language priors conflict with counterfactual visual evidence, how often do they override the visual evidence?

    \item[] \textbf{RQ6: Language-aligned Spatial Bias.}
    What proportion of spatial bias aligns with erroneous language priors, and how much remains non-language-aligned?
\end{itemize}

% \begin{itemize}[leftmargin=*]
%     \item[] \textbf{RQ1: Spatial Reasoning Performance.}
%     How accurately and consistently do VLMs reason across original and counterfactual visual conditions?

%     \item[] \textbf{RQ2: Counterfactual Failure.}
%     How often do VLMs fail under counterfactual interventions, and how much of these failures can be distinguished as bias-related versus non-bias errors?

%     \item[] \textbf{RQ3: Spatial Bias Prevalence.}
%     How frequently do VLMs retain or follow prior-consistent spatial predictions despite contradictory counterfactual evidence?

%     \item[] \textbf{RQ4: Language-prior Prevalence.}
%     How frequently do VLMs exhibit language priors toward the original spatial answer in the absence of visual evidence?

%     \item[] \textbf{RQ5: Language-prior Dominance.}
%     When language priors conflict with counterfactual visual evidence, how often do they override the visual evidence?

%     \item[] \textbf{RQ6: Language-aligned Spatial Bias.}
%     How frequently do spatial biases align with erroneous language priors, and how much bias remains non-language-aligned?
% \end{itemize}

\textbf{Metric Overview.}
The designed metrics form a hierarchical diagnosis from \emph{spatial capability} to \emph{counterfactual failure}, \emph{spatial bias}, and finally \emph{language-prior attribution}.
For \textbf{RQ1}, $Acc^{O}$, $Acc^{CF}$, $pAcc$, and $mAcc$ establish overall spatial reasoning accuracy and consistency.
Building on samples correctly answered in the original condition, \textbf{RQ2} uses Counterfactual Error Rate (CER) to quantify failures induced by counterfactual changes, with Non-Bias Error Rate (NBER) isolating residual errors beyond identified bias.
\textbf{RQ3} further characterizes these systematic failures through Prior Retention Rate (PRR), which captures persistence of the original answer, and Bias Rate (BR), which measures overall spatial bias.
Finally, \textbf{RQ4--RQ6} trace the role of language priors: Language Prior Dependence (LPD) measures their prevalence, Text Override Rate (TOR) measures their dominance when language and visual evidence conflict, and Language-aligned Bias Rate (LBR) measures their manifestation as spatial bias.
Thus, LPD, TOR, and LBR respectively characterize whether a language prior exists, whether it overrides conflicting visual evidence, and whether it manifests as spatial bias.
When $\mathrm{LPD}=1$, all eligible samples constitute language--vision conflicts, yielding $\mathrm{TOR}=\mathrm{LBR}$.
Detailed definitions and calculations are provided in Table~\ref{tab:metrics}.

% \textbf{Metric Overview.}
% For \textbf{RQ1}, we use original accuracy ($Acc^{O}$), counterfactual accuracy ($Acc^{CF}$), pair accuracy ($pAcc$), and mean accuracy ($mAcc$) to measure spatial capability and consistency.
% For \textbf{RQ2}, Counterfactual Error Rate (CER) measures failures on eligible counterfactual samples, while Non-Bias Error Rate (NBER) captures the residual errors not identified as spatial bias.
% For \textbf{RQ3}, Prior Retention Rate (PRR) quantifies the tendency to preserve the original answer after the spatial ground truth changes, whereas Bias Rate (BR) measures the overall prevalence of identified spatial bias.
% For \textbf{RQ4--RQ6}, Language Prior Dependence (LPD) measures the prevalence of original-answer language priors, Text Override Rate (TOR) measures the susceptibility to language-over-vision override under direct conflict, and Language-aligned Bias Rate (LBR) measures the prevalence of spatial errors aligned with erroneous text-only predictions.
% The remaining non-language-aligned bias is given by
%     $\mathrm{NLBR}=\mathrm{BR}-\mathrm{LBR}$.
% %
% Importantly, LBR and TOR capture different aspects of language-prior effects: LBR measures their overall manifestation as spatial bias, whereas TOR conditions specifically on language--vision conflicts and measures how often language dominates.
% When the text-only prediction equals the original answer for all eligible samples, i.e., $\mathrm{LPD}=1$, every eligible sample constitutes a language--vision conflict and thus $\mathrm{TOR}=\mathrm{LBR}$.
% Detailed metric calculations are summarized in Table~\ref{tab:metrics}.


% \subsection{Metrics Beyond Accuracy}

% We design evaluation metrics beyond accuracy for deeper analysis and understanding of the spatial bias and other errors by addressing the following research questions (RQ):
%     \begin{itemize}[leftmargin=*]
%         \item[] \textbf{RQ1: Spatial Reasoning Performance.} Can the model answer correctly? How accurately and consistently do VLMs perform spatial reasoning across original and counterfactual visual conditions?
%         \item[] \textbf{RQ2: Counterfactual Failure.} How frequently do VLMs fail under counterfactual visual interventions, and to what extent are these failures associated with spatial bias?
%         \item[] \textbf{RQ3: Spatial Bias Prevalence.} Does bias occur? How prone is the model to persisting in its original answer after the visual ground truth changes? 
%         \item[] \textbf{RQ4: Language-prior Prevalence.} How prevalent are language priors in spatial reasoning? To what extent do VLMs exhibit language priors toward the original spatial answer in the absence of visual evidence?
%         \item[] \textbf{RQ5: Language-prior Dominance.} How strongly does language override vision? When language priors directly conflict with visual facts, how prone is the model to prioritizing language over vision?
%         \item[] \textbf{RQ6: Language-aligned Spatial Bias.} Is the bias aligned with language prior? Among these spatial biases, what proportion across the overall dataset manifests as language-aligned bias versus non-textual biases (e.g., visual, alignment, or reasoning failures)?
%     \end{itemize}

% \textbf{Metric Overview.} 
% $Acc^O$ for original accuracy.
% $Acc^{CF}$ for counterfactual accuracy.
% $pAcc$ denotes Pair accuracy for pairwise consistency.
% $mAcc$ denotes mean accuracy for overall accuracy.
% BR for bias detection.
% TOR for modality competition. TOR for prior dominance. To quantify the degree of language-vision conflict, we propose a metric named text override rate (TOR)
% LBR for language-prior bias attribution and prevalence.
% Specifically, LBR quantifies the prevalence of language-aligned spatial bias, whereas TOR measures the susceptibility of the model to language priors when linguistic preference conflicts with counterfactual visual evidence. 
% Naturally, the non-language bias rate follows $NLBR=BR-LBR$.
% LPD for language-prior prevalence.
% Note that in cases where all $\hat y^T_i=y^O_i$, meaning dataset with high LPD, TOR equals LBR. This indicates that the language prior conflicts with the counterfactual visual evidence across all eligible samples, such that the overall language-bias rate is determined solely by the model’s susceptibility to language-over-vision override. 
% %
% The detailed introduction of each metric is illustrated in Table \ref{tab:metrics}.

\textbf{Diagnostic Notations.}
Let $\mathds{1}(\cdot)$ denote the indicator function. We first define the flipped-answer set $\mathcal{D}_{\mathrm{flip}}=\{i:(I_i,q_i)\in\mathcal{V},\ y_i^{CF}\neq y_i^O\}$, which contains samples whose ground-truth answers change after counterfactual editing. For bias diagnosis, we further restrict to the eligible set $\mathcal{E}=\{i\in\mathcal{D}_{\mathrm{flip}}:\hat y_i^O=y_i^O\}$, thereby excluding samples that are already incorrect on the original input. We denote the text-only prediction as $\hat y_i^T=\mathcal{M}(q_i)$, obtained without image input. The overall bias set is defined as $\mathcal{B}=\mathcal{B}^O\cup\mathcal{B}^L$, where $\mathcal{B}^O=\{i\in\mathcal{D}_{\mathrm{flip}}:\hat y_i^{CF}=y_i^O\}$ denotes original-answer retention bias, and $\mathcal{B}^L=\{i\in\mathcal{D}_{\mathrm{flip}}:\hat y_i^{CF}=\hat y_i^T\neq y_i^{CF}\}$ denotes language-aligned bias. Finally, we define the language--vision conflict set as $\mathcal{C}=\{i\in\mathcal{E}:\hat y_i^T\neq y_i^{CF}\}$.

% Let $\mathds{1}(\cdot)$ be the indicator function.
% %
% For clarity, we denote $\hat y^T_i=\mathcal{M}(q_i)$ as the text-only model's predicted answer without image input.
% %
% Specifically, we define $\mathcal{D}_{\mathrm{flip}}=\{i: y^{CF}_i\neq y^O_i, (I_i,q_i)\in\mathcal{V}\}$ with flipped GT answers for original and edited images to ensure valid calculation of bias rate. 
% %
% Then, we define the bias event set as $\mathcal{B}=\mathcal{B}^O\cup\mathcal{B}^L$, where $\mathcal{B}^O=\{i\in\mathcal{D}_{\mathrm{flip}}:\hat y^{CF}_i=y_i^O\}$ denotes the original retention bias set and $\mathcal{B}^L=\{i\in\mathcal{D}_{\mathrm{flip}}: \hat y^{CF}_i=\hat y_i^T\neq y^{CF}_i\}$ is the language-aligned bias set.
% %
% For simplicity, we define an eligible set as $\mathcal{E}=\{i\in\mathcal{D}_{\mathrm{flip}}: \hat y^{O}_i=y^O_i\}$ for bias diagnosis of eligible samples, and abbreviate original and counterfactual as O and CF, respectively. Also, we define a language–vision conflict set as $\mathcal{C}=\{i\in\mathcal{E}: \hat y_i^T\neq y_i^{CF}\}$.

\input{tables/metrics}



==> sections/Bias_reason.tex <==
\section{Reason of Bias Emergence}
\label{bias_reason}
% why spatial bias exist?

data layer

model layer



==> sections/Discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\textbf{The prior knowledge trap.}
Our findings reveal a fundamental tension between prior knowledge and perceptual grounding. We term this the \textbf{prior knowledge trap}: priors can support reasoning under incomplete, noisy, or ambiguous observations, but become harmful when they override reliable visual evidence. Thus, the issue is not prior knowledge itself, but its miscalibrated use. Robust spatial intelligence should therefore emphasize \emph{prior calibration}---relying on priors when evidence is weak while yielding to observations when the two conflict. This perspective may extend beyond spatial bias to other multimodal biases, where learned regularities are useful only when appropriately conditioned on current evidence.

\textbf{Implications for 3D generation and reconstruction.}
The same trade-off is particularly relevant to 3D generation, reconstruction, and scene completion, where observations are often sparse and under-constrained. Spatial priors can help infer unobserved geometry and produce plausible completions, but overly strong priors may favor canonical viewpoints, common scales, or familiar layouts over atypical yet valid evidence. Spatial bias therefore suggests a broader tension between \emph{plausibility} and \emph{evidence fidelity}, which deserves further study in generative spatial models.

\textbf{Limitations and future work.}
Our benchmark focuses on controlled counterfactual VQA and does not yet cover the full diversity of embodied interaction. Future work will extend to broader agents and scenarios, including autonomous vehicles, robotic manipulators, mobile robots, and humanoids, as well as dynamic scenes, temporal reasoning, multi-view perception, and physical interaction. We also plan to study spatial bias beyond image-based VLMs, including video-language models, unified multimodal models, vision-language-action models, multimodal agents, and world-model-based systems. Finally, our current framework diagnoses bias primarily from observable behavior; combining counterfactual probing with representation analysis, uncertainty estimation, causal intervention, and mechanistic interpretability may further reveal where spatial priors arise and how they influence multimodal reasoning.

% \section{Discussion}
% \label{sec:discussion}

% \textbf{The prior knowledge trap: when does a useful prior become a bias?}
% Although spatial bias is undesirable when it causes a model to ignore contradictory visual evidence, our findings also reveal a broader tension between prior knowledge and perceptual grounding.
% We term this phenomenon the \textbf{prior knowledge trap}: the same prior that enables effective reasoning under incomplete, noisy, or ambiguous observations may become harmful once it dominates reliable visual evidence.
% Thus, the fundamental problem is not the existence of prior knowledge itself, but its \emph{miscalibrated use}.
% When observations are uncertain, learned spatial priors may provide useful regularization and compensate for missing information; when reliable evidence is available, however, persistent reliance on these priors can lead to systematic spatial bias.
% In short, \emph{a prior is useful when it complements uncertain evidence, but becomes a bias when it overrides reliable evidence}.
% This suggests that robust spatial intelligence should focus on \emph{prior calibration} rather than indiscriminate prior suppression.

% \textbf{Useful priors for uncertain embodied reasoning.}
% Many embodied tasks are inherently affected by partial observability, occlusion, sensor noise, and incomplete geometric information.
% Under such conditions, prior knowledge about object layouts, relative scale, physical accessibility, viewpoint relations, and common spatial configurations can facilitate plausible inference when direct observations are insufficient.
% Such priors may therefore benefit tasks requiring empirical judgment or spatial completion.
% However, their utility depends critically on whether the model can adapt the strength of prior reliance to the confidence of current observations.
% An ideal embodied model should exploit priors when perceptual evidence is weak, while yielding to direct visual evidence when the two disagree.

% \textbf{Potential influence on 3D generation and reconstruction.}
% The same perspective naturally extends to 3D generation, reconstruction, and scene completion, where observations are frequently sparse and the underlying solution space is highly under-constrained.
% Spatial priors may help infer unobserved geometry, complete occluded regions, and generate structurally plausible 3D scenes from incomplete views.
% At the same time, overly dominant priors may bias generated content toward canonical viewpoints, common object scales, familiar layouts, or frequently observed spatial arrangements, even when the available evidence supports an atypical but valid configuration.
% Therefore, spatial priors can improve \emph{plausibility} while potentially reducing \emph{evidence fidelity}.
% Although generative 3D modeling is beyond the direct scope of this work, our findings suggest that spatial-bias analysis may provide a useful perspective for studying this trade-off in future spatial generative models.

% \textbf{Beyond spatial-bias removal.}
% Our results further suggest that spatial-bias mitigation should not necessarily aim to eliminate all prior-driven behavior.
% A more desirable objective is to improve the model's ability to decide \emph{when} and \emph{how strongly} prior knowledge should influence prediction.
% This perspective may also generalize beyond spatial bias.
% Across social, visual, and spatial settings, learned priors can support generalization when they capture useful regularities, yet become problematic when applied rigidly or remain insensitive to contradictory evidence.
% Accordingly, an important direction for future multimodal systems is to explicitly model the balance between prior confidence and observation reliability.

% \textbf{Limitations and future work.}
% This study focuses on a controlled set of embodied spatial reasoning tasks and counterfactual VQA pairs, which enables precise diagnosis but does not yet cover the full diversity of real-world embodied interaction.
% Future work will extend the benchmark toward broader application scenarios and more general embodied spatial tasks, including aerial drones, autonomous vehicles, robotic manipulators, mobile robots, and humanoid agents.
% Such extensions can further incorporate dynamic scenes, temporal reasoning, multi-view observations, physical interaction, and action-conditioned spatial understanding, thereby evaluating whether the identified bias patterns persist under more realistic perception--reasoning--action loops.

% Our current investigation also primarily targets VLM-based spatial reasoning.
% An important future direction is to study whether similar spatial biases emerge in more general multimodal foundation models, including video-language models, unified multimodal large language models, vision-language-action models, multimodal agents, and generative or world-model-based systems.
% These models integrate richer temporal, action, and generative signals than conventional VLMs, but may still inherit or amplify spatial priors from large-scale pre-training.
% Extending spatial-bias diagnosis beyond static image--text reasoning will therefore be essential for understanding whether systematic spatial preferences constitute a broader property of multimodal intelligence.

% Finally, the current diagnostic framework mainly identifies bias through observable prediction patterns and their alignment with prior responses.
% While this provides a practical and interpretable behavioral diagnosis, it does not fully establish the internal causal mechanisms responsible for each bias type.
% Future work could combine counterfactual probing with representation analysis, uncertainty estimation, causal intervention, and mechanistic interpretability to better localize where spatial priors arise and how they propagate through multimodal reasoning.
% Together, these directions may support the development of embodied models that are not only more accurate, but also more adaptive, evidence-sensitive, and reliable under spatial uncertainty.


% \textbf{influence on 3D generation}

% Despite the probing framework and corresponding mitigation techniques of spatial bias in VLMs with adverse impacts on embodied applications, this work also provides another interesting alternative perspective on the positive sides of spatial bias, which we call the \textbf{prior knowledge trap}.

% % beneficial bias rate
% % \begin{equation}
% %     bBR=
% % \end{equation}
% Although bias sounds like a derogatory term, is bias always a bad thing?

% Which kind of prior knowledge may be helpful?

% Is bias rather an advantage for problem with empirical judgment needs?

% And this perspective is of generality across all the bias in VLMs, including social, visual, and spatial bias. 



==> sections/Introduction.tex <==
\section{Introduction}
\label{sec:intro}

\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{figs/intro.pdf}
    \caption{\textbf{Motivation of spatial bias in VLMs.} (a) A representative original--counterfactual pair shows that VLMs may retain the original answer despite recognizing the visual change, indicating a potential spatial bias.
    % ; gradient-response heatmaps illustrate the model's attended regions. 
    (b) Comparison of original (O), counterfactual (CF), and pair accuracy (correct on both O and CF) reveals substantial performance degradation under counterfactual interventions. (c) Model bias rate across six spatial reasoning categories.
}
    \label{fig:intro}
    \vspace{-15pt}
\end{figure}

Spatial reasoning is a fundamental capability for embodied intelligence, as an agent needs to understand \emph{where} objects are, \emph{how} they are spatially related, and \emph{whether} an action is geometrically and physically feasible before interacting with the environment.
Such capabilities underpin a wide range of embodied tasks, including object manipulation, navigation, autonomous driving, and robotic interaction~\cite{song2025robospatial,zhou2025physvlm,wang2025metavqa}.
Unlike conventional visual recognition, embodied spatial reasoning requires models to move beyond semantic recognition toward structured reasoning about relative position, orientation, distance, reference frames, accessibility, and interaction constraints.
Failures in these capabilities can directly propagate to downstream decisions, making reliable spatial reasoning a prerequisite for robust embodied agents.

Vision-Language Models (VLMs) have emerged as a promising foundation for such embodied spatial intelligence.
% Early large-scale multimodal models established powerful interfaces between pretrained visual encoders and language models~\cite{alayrac2022flamingo,li2023blip2,liu2023llava}, enabling visual question answering, instruction following, and open-ended multimodal reasoning.
% Recent research focus has increasingly shifted from general visual-language understanding toward explicit spatial and embodied reasoning.
SpatialVLM~\cite{chen2024spatialvlm} scales spatial supervision to improve qualitative and quantitative 3D reasoning; RoboSpatial~\cite{song2025robospatial} introduces robot-oriented spatial supervision involving multiple reference frames and object--space relations; PhysVLM~\cite{zhou2025physvlm} explicitly incorporates physical reachability into embodied reasoning. Recent work further extends VLMs toward multi-view spatial reasoning and 3D-aware embodied control~\cite{jeong2026xvr,nikolov2026spear}.
These advances reflect a clear technical trend from {generic multimodal understanding} toward {spatially grounded, geometry-aware, and action-oriented intelligence}.

Despite this rapid progress, current research predominantly asks a capability-oriented question:
\emph{Can VLMs reason spatially?}
Existing benchmarks typically evaluate spatial relations, egocentric understanding, metric estimation, reference-frame reasoning, or embodied interaction primarily through visual-question answering (VQA) accuracy~\cite{du2024embspatial,chen2024spatialvlm,song2025robospatial}.
These studies have revealed that contemporary VLMs remain imperfect at spatial reasoning, but an incorrect answer alone provides limited insight into \emph{how} a model fails.
In particular, two models with similar accuracy may exhibit fundamentally different error behaviors: one may make relatively unstructured mistakes, whereas another may repeatedly favor a particular spatial configuration even when contradictory visual evidence is explicitly provided, as illustrated in Fig.~\ref{fig:intro}.
Recent diagnostic evidence has begun to show that spatial VLMs can remain highly consistent while being incorrect, suggesting insufficient sensitivity to spatial evidence~\cite{bhat2026viewdiag}.
However, whether such failures constitute a broader and systematic \emph{spatial bias}, how this bias manifests across different embodied spatial tasks, and what priors are associated with it remain largely unexplored.

This gap is distinct from the bias and reliability failures widely studied in VLMs.
Most existing bias studies focus on \emph{social or demographic bias}, including gender, race, age, profession, and other human attributes~\cite{wang2026vlbiasbench,huang2025visbias,howard2024socialcounterfactuals}, as illustrated in Fig.~\ref{fig:bias_comparison}.
More recent studies investigate \emph{visual bias}, showing that learned semantic or memory priors can override current visual evidence, even under controlled counterfactual modifications or visual illusions~\cite{vo2026vlmsbiased,sun2026vlms}.
Another major line examines \emph{visual hallucination}, where models produce objects or statements unsupported by the image~\cite{li2023pope,guan2024hallusionbench}; HallusionBench~\cite{guan2024hallusionbench} further distinguishes failures associated with language priors from visual misinterpretation.
While these studies expose important limitations of VLMs, systematic preferences in \emph{spatial reasoning} remain underexplored.
For embodied intelligence, such a distinction is critical: a model may correctly recognize scene content without conventional object hallucination, yet still systematically misjudge relative position, direction, distance, viewpoint, or feasible actions.

% This gap is distinct from the forms of bias and reliability failure that have received substantial attention in existing VLM research.
% Most VLM bias studies focus on \emph{social or demographic bias}, such as biases related to gender, race, age, profession, and other human attributes~\cite{wang2026vlbiasbench,huang2025visbias,howard2024socialcounterfactuals}, as shown in Fig.~\ref{fig:bias_comparison}\footnote{The data samples for social and visual bias are respectively sourced from \cite{huang2025visbias} and \cite{vo2026vlmsbiased}.}.
% Another major line of research investigates \emph{visual hallucination}, where models generate objects or statements unsupported by the image~\cite{li2023pope,guan2024hallusionbench}.
% HallusionBench~\cite{guan2024hallusionbench} further distinguishes failures associated with language priors from visual misinterpretation.
% While these studies expose important limitations of VLMs, they do not directly address systematic preferences in \emph{spatial reasoning}.
% For embodied intelligence, such a distinction is crucial: a model may correctly recognize all objects in a scene and generate no conventional object hallucination, yet still systematically infer an incorrect relative position, direction, distance, viewpoint relation, or feasible action.

\begin{figure}[t]
    \centering
    \includegraphics[width=1\linewidth]{figs/bias_comparison.pdf}
    \caption{ \textbf{Investigation scope.} Left: Comparison of spatial bias with previously studied social and visual biases~\cite{huang2025visbias,vo2026vlmsbiased}. Right: Distinctions and overlaps among model error, hallucination, and bias.}
    \vspace{0.3em}
    \label{fig:bias_comparison}
    \vspace{-10pt}
\end{figure}

In this work, we shift the evaluation perspective from \emph{spatial reasoning accuracy} to \emph{spatial error tendency}.
We study whether VLMs systematically favor particular spatial configurations or prior-consistent answers despite visual evidence supporting an alternative configuration.
We refer to this phenomenon as \textbf{spatial bias}: a systematic tendency of a VLM to produce prior-aligned spatial predictions that are insufficiently responsive to the spatial evidence presented in the current visual input.
Rather than treating every spatial error as bias, our diagnostic framework explicitly distinguishes structured bias-related failures from general prediction errors.
This distinction allows us to investigate not only \emph{whether} a model is wrong, but also \emph{whether its errors exhibit systematic directional tendencies and what prior signals are associated with them}.

To probe such behavior, we adopt a \textbf{counterfactual testing paradigm}.
Counterfactual reasoning has previously been used to expose language shortcuts in VQA and social biases in VLMs~\cite{niu2021counterfactual,howard2024socialcounterfactuals}.
Here, we extend this principle to embodied spatial reasoning by constructing paired original and counterfactual visual scenes that preserve the question and non-target semantic content while selectively modifying task-relevant spatial evidence.
If a model is genuinely grounded in the visual scene, its prediction should change whenever the underlying spatial ground truth changes.
Conversely, retaining a prior answer or following an erroneous text-only preference despite contradictory counterfactual evidence provides a controlled probe of systematic spatial bias.
This paired design therefore enables us to separate basic task capability, counterfactual failure, prior retention, language-aligned bias, and residual non-bias errors within a unified diagnostic framework.

Based on this perspective, we systematically investigate three questions:
\emph{(i)} how prevalent spatial bias is across contemporary VLMs and embodied spatial tasks;
\emph{(ii)} how such bias differs from ordinary spatial reasoning errors and interacts with language priors; and
\emph{(iii)} whether common prompting and training strategies can mitigate these systematic tendencies.
Our study reveals that spatial errors in VLMs are far from arbitrary: under controlled counterfactual interventions, a considerable fraction of failures follow identifiable prior-retention or language-aligned patterns, motivating evaluation beyond conventional accuracy.
%
Our main contributions are fivefold:
\begin{itemize}[nosep,leftmargin=*]
    \item \textbf{We identify and characterize spatial bias in VLMs.}
    We formulate spatial bias as a distinct failure mode in spatial reasoning and introduce a taxonomy covering its manifestations across spatial tasks and potential prior sources.

    \item \textbf{We construct a counterfactual benchmark for spatial-bias evaluation.}
    To the best of our knowledge, it is the \textbf{first} benchmark explicitly designed for spatial-bias diagnosis using paired original--counterfactual embodied VQA examples, covering 24 task--source categories under controlled spatial interventions.

    \item \textbf{We develop a multi-stage framework that disentangles spatial bias from generic spatial errors.} Beyond aggregate accuracy, the framework decomposes counterfactual failures into prior-retention bias, language-aligned bias, and residual non-bias errors, with our designed dedicated metrics for quantifying bias prevalence and language-prior effects.

    \item \textbf{We conduct extensive evaluations across diverse VLMs.}
    Our study reveals widespread spatial bias and analyze its variation across model families, spatial tasks, and bias sources, as well as its sensitivity to input organization and background information.

    \item \textbf{We investigate bias mitigation strategies at both inference and parameter levels.} We evaluate zero-shot intervention, chain-of-thought incorporation, few-shot prompting, and supervised fine-tuning, showing that prompting yields limited or model-dependent gains, whereas supervised fine-tuning provides substantially more consistent bias reduction.
\end{itemize}

% Our main contributions are fivefold:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{We identify and systematically characterize spatial bias in VLMs.}
%     We formulate spatial bias as a distinct failure mode of embodied spatial reasoning and develop a taxonomy according to its manifestations across spatial tasks and its potential prior sources, distinguishing systematic bias from generic reasoning errors.

%     \item \textbf{We construct a dedicated counterfactual benchmark for spatial-bias evaluation.}
%     To the best of our knowledge, it is the first benchmark explicitly designed to diagnose spatial bias through paired original--counterfactual embodied VQA examples.
%     The benchmark covers 24 categories of spatial reasoning tasks and enables controlled evaluation under changes in task-relevant spatial evidence.

%     \item \textbf{We propose a multi-stage spatial-bias diagnostic framework beyond accuracy.}
%     The framework progressively analyzes basic spatial capability, counterfactual failures, prior-retention behavior, language-aligned bias, and non-bias errors.
%     We further introduce a systematic suite of diagnostic metrics to quantify not only the prevalence of spatial bias but also its dependence on language priors and its distinction from general errors.

%     \item \textbf{We conduct extensive evaluations across diverse mainstream VLM families.}
%     Our experiments reveal the widespread existence of spatial bias and analyze its relationship with model families, spatial task categories, and potential bias sources.
%     We further investigate how input and background configurations affect spatial-bias behavior.

%     \item \textbf{We systematically investigate strategies for mitigating spatial bias.}
%     We evaluate zero-shot linguistic intervention, chain-of-thought prompting, few-shot assistance, and supervised fine-tuning.
%     The results show that prompting-based interventions provide limited or model-dependent benefits, whereas supervised fine-tuning can substantially reduce spatial bias, highlighting the importance of explicitly bias-aware training signals.
% \end{itemize}


% Spatial reasoning is significant in embodied tasks applications.

% The important role of VLMs in intelligent spatial reasoning for embodied robot tasks and the techniques trend.

% However, a critical limitation called spatial bias of VLM in spatial reasoning is discovered, which is not investigated before, since previous work mainly focus on social bias and visual hallucination.

% Existing studies have investigated whether VLMs can reason spatially, but not whether they reason spatially in a systematically biased manner.

% We shift the focus from spatial reasoning accuracy to spatial error tendency, investigating whether VLMs systematically favor certain spatial configurations despite comparable semantic content.

% Specifically, we adopt the counterfactual test to probe spatial bias.

% The main contributions are fivefold:
% \begin{itemize}[leftmargin=*]
%     \item We discover the phenomenon of spatial bias in VLMs and categorize it according to model's different manifestations for various spatial tasks and potential bias sources. 
%     \item We build the first spatial bias benchmark composed of original-counterfactual embodied VQA pairs with 24 categories to evaluate VLM's performance on embodied spatial reasoning tasks.
%     \item We propose a novel multi-stage bias diagnostic framework to dig out the spatial bias and error in VLMs and its dependency on language prior. We also design a systematic set of evaluation metrics beyond accuracy to better analyze the emergence reason of spatial bias.
%     \item We conduct experiments on different mainstream VLM families to show the common issues of spatial bias, there relationships with different spatial tasks and bias reasons, and further analyze the influence of various input configurations and background information.
%     \item We test several bias mitigation methods including linguistic intervention, CoT prompting, few-shot assistance, and fine-tuning with positive-negative sample signals. Results find that SFT effectively reduce the VLMs' spatial bias.
% \end{itemize}



==> sections/Related_work.tex <==
\section{Related Work}
\label{sec:related_work}

\textbf{Bias in VLMs.}
Bias in vision-language models (VLMs) has been mainly studied as \emph{social bias} and, more recently, \emph{visual bias}. 
VLBiasBench~\cite{wang2026vlbiasbench} systematically evaluates demographic biases across multiple categories and interaction settings, while VisBias~\cite{huang2025visbias} further distinguishes explicit and implicit social biases in judgment, description, and assistance tasks. 
These works reveal persistent stereotypes in VLMs but primarily focus on human-related attributes. 
Recent studies extend bias analysis to visual perception itself. Vo et al.~\cite{vo2026vlmsbiased} use counterfactual images to show that VLMs often favor pretrained semantic priors over observed visual evidence, especially in object identification and counting. 
However, existing studies largely target demographic, semantic, or object-level priors, leaving systematic preferences over \emph{spatial configurations}, such as position, direction, distance, viewpoint, and relation, underexplored. 
This motivates our study of \emph{spatial bias}, compared with prior bias settings in Fig.~\ref{fig:bias_comparison}\footnote{The data samples for social and visual bias are respectively sourced from \cite{huang2025visbias} and \cite{vo2026vlmsbiased}.}.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/bias_comparison.pdf}
    \caption{Comparison of our work on spatial bias in VLMs with existing work on social and visual bias (left), and the relationships among model error, hallucination, and bias (right).}
    \label{fig:bias_comparison}
\end{figure}

\textbf{Hallucination in VLMs.}
Hallucination refers to VLM outputs that are inconsistent with visual evidence. 
Early work mainly studies object hallucination. LURE~\cite{zhou2024lure} analyzes factors such as object co-occurrence priors and generation uncertainty, and mitigates hallucination through post-hoc revision. 
AMBER~\cite{wang2024amber} extends evaluation to object existence, attributes, and relations, while HallusionBench~\cite{guan2024hallusionbench} distinguishes language-induced hallucination from visual misunderstanding using controlled image--question pairs. 
Mitigation methods further evolve toward inference-time intervention: OPERA~\cite{huang2024opera} penalizes over-reliance on visual summary tokens, whereas Woodpecker~\cite{yin2024woodpecker} verifies and corrects generated claims against visual evidence. 
Despite this progress, hallucination studies mainly characterize whether predictions contradict the image, rather than whether such errors exhibit systematic spatial tendencies. 
Our work therefore focuses on structured spatial preferences underlying repeated errors, rather than isolated hallucinated outputs.

\textbf{Spatial Reasoning with VLMs.}
Spatial reasoning in VLMs involves localization, spatial relations, metric estimation, orientation, and viewpoint transformation. 
SpatialVLM~\cite{chen2024spatialvlm} improves quantitative spatial reasoning by constructing large-scale 3D spatial VQA data with explicit supervision on distance and size. 
VSI-Bench~\cite{yang2025thinking} further evaluates scene-level spatial understanding from egocentric videos, including layout memory, distance estimation, and egocentric--allocentric transformation, showing that spatial reasoning remains challenging for current multimodal models. 
These studies have motivated geometry-grounded representations using depth, 3D reconstruction, and structured spatial cues. 
However, existing benchmarks mainly measure \emph{whether} models reason correctly, while paying limited attention to the \emph{direction and distribution} of their errors. 
Our work complements this line by investigating whether VLM spatial reasoning exhibits systematic and persistent bias.

% \subsection{Spatial Hallucination}

==> sections/Spatial_bias.tex <==
\section{Spatial Bias}
\label{sec:spatial_bias}

\textbf{Investigation Scope.}
This work focuses on spatial bias in VLMs and distinguish it from several related phenomena.
Unlike \emph{social bias}, which concerns demographic or social associations, and broader \emph{visual bias}, which may arise from appearance, context, or visual-semantic priors, our study specifically targets systematic tendencies in spatial reasoning.
Spatial bias is also different from \emph{spatial error}, which includes any incorrect spatial prediction, and from \emph{hallucination}, which refers to outputs unsupported by visual evidence.
Likewise, limited spatial reasoning capability concerns overall task performance, whereas spatial bias concerns the \emph{structure and direction} of errors.
These phenomena may overlap but are not equivalent, as illustrated in Fig.~\ref{fig:bias_comparison}.

% \textbf{Investigation Scope.}
% This work studies \emph{spatial bias} in VLMs, i.e., systematic preferences that emerge when models interpret spatial information such as depth and scale, geometric structure, spatial relations, and viewpoint or orientation.
% Spatial bias differs from several related concepts.
% \emph{Social bias} concerns stereotypical or unfair associations involving demographic or social attributes, whereas \emph{visual bias} generally refers to systematic preferences induced by visual appearance, context, or learned visual-semantic priors.
% In contrast, spatial bias specifically concerns systematic distortions in the interpretation of spatial configurations and relations.
% It is also distinct from a generic \emph{spatial error}, which includes any incorrect prediction, and from \emph{hallucination}, which broadly denotes outputs unsupported by the input evidence.
% Similarly, limited spatial reasoning capability reflects overall task performance, while spatial bias concerns the \emph{structure and direction} of errors.
% %
% An error denotes an incorrect prediction; hallucination denotes inconsistency with visual evidence; bias refers to a systematic directional tendency across controlled examples. These phenomena may overlap but are not equivalent.
% %
% Accordingly, rather than asking only whether a VLM reasons spatially correctly, we investigate whether its errors systematically favor prior-consistent spatial interpretations despite conflicting visual evidence (Fig.~\ref{fig:bias_comparison}).

\textbf{Definition.}
We formally define spatial bias in VLMs as follows:
\begin{tcolorbox}[
    colback=gray!5!white,
    colframe=black!75,
    boxrule=0.8pt,
    arc=4pt,
    left=6pt, right=6pt, top=6pt, bottom=6pt,
    coltitle=white,
    colbacktitle=black,
    fonttitle=\bfseries,
    title=Definition of Spatial Bias
]
\emph{Spatial bias} is a systematic and non-random tendency of a VLM toward particular spatial configurations, relations, or interpretations that are inconsistent with the current visual evidence, typically reflecting the influence of learned priors over spatial observations.
\end{tcolorbox}


% \textbf{Investigation Scope.}
% This work investigates \emph{spatial bias} in VLMs, defined as systematic and directional preferences that arise when models perceive and reason about spatial information, including depth and scale, geometric structure, spatial position and relations, and viewpoint and orientation. Unlike a \emph{spatial error}, which denotes any incorrect prediction, spatial bias reflects structured tendencies that persist across samples; unlike \emph{hallucination}, which describes outputs unsupported by visual evidence, spatial bias characterizes systematic preferences that may contribute to such failures (Fig.~\ref{fig:bias_comparison}, right). It is also distinct from limited spatial reasoning capability, which concerns overall task performance rather than the structure and direction of errors. Accordingly, our goal is not merely to measure whether VLMs make spatial mistakes, but to identify whether they systematically favor certain spatial interpretations despite conflicting visual evidence, thereby revealing failure patterns that can be obscured by aggregate accuracy.

% % \textbf{Investigation Scope.}
% % This work focuses on \emph{spatial bias} in vision-language models (VLMs), namely systematic preferences that emerge when models perceive, interpret, and reason about spatial information. 
% % We investigate biases related to spatial position, relative relations, geometric structure, depth and scale, viewpoint and orientation, and spatially grounded actions. 
% % These factors are fundamental to visual understanding and embodied intelligence, yet errors in them can directly affect localization, scene understanding, navigation, and decision making.

% % Spatial bias is related to, but distinct from, generic model error and hallucination. 
% % A \emph{model error} only indicates that a prediction is incorrect, whereas spatial bias emphasizes a persistent and directional tendency across samples. 
% % A \emph{hallucination} refers to an output that is unsupported by the visual evidence, while spatial bias describes the systematic preference that may underlie such failures. 
% % Therefore, not every spatial error constitutes a bias, and not every hallucination is caused by spatial bias, as depicted in Fig.~\ref{fig:bias_comparison} (right).

% % Our goal is thus not merely to measure whether VLMs make spatial mistakes, but to identify whether these mistakes exhibit stable and structured tendencies. 
% % Understanding such biases is important for revealing hidden failure patterns that may be obscured by aggregate accuracy, and for improving the reliability of VLMs in spatially demanding and embodied applications.

% % Spatial bias arises when the prediction change is systematically inconsistent with the change in visual evidence. 
% % This definition distinguishes spatial bias from several related concepts. 
% % A \emph{spatial error} refers to any incorrect prediction and may occur randomly, whereas spatial bias requires a consistent directional tendency across examples. 
% % A \emph{hallucination} describes an output unsupported by the image, while spatial bias characterizes the systematic preference that may contribute to such hallucinations. 
% % Similarly, poor spatial reasoning capability indicates limited task performance in general, whereas spatial bias specifically concerns the \emph{structure and direction} of the resulting errors.

% % Therefore, our objective is not only to measure whether VLMs make spatial mistakes, but to determine whether they \emph{prefer certain spatial interpretations over others in a systematic manner}.

% \textbf{Definition.}
% Specifically, we define the spatial bias of VLMs as follows. 
% \begin{tcolorbox}[
%     colback=gray!5!white,  % 背景颜色
%     colframe=black!75,     % 边框颜色
%     boxrule=0.8pt,         % 边框粗细
%     arc=4pt,               % 圆角弧度
%     left=6pt, right=6pt, top=6pt, bottom=6pt, % 内边距,
%     coltitle=white,          % 标题文字颜色（白色）
%     colbacktitle=black,      % 标题栏背景色
%     fonttitle=\bfseries,     % 标题文字加粗
%     title=Definition of spatial bias
% ]
% Spatial bias refers to a systematic and non-random preference of a VLM toward particular spatial configurations, relations, or interpretations that cannot be fully explained by the visual evidence, resulting in prediction results systematically follows a prior inconsistent with the current visual evidence.
% \end{tcolorbox}
%

% \textbf{Problem Formulation.}
% Spatial bias arises when the prediction change is systematically inconsistent with the change in visual evidence. 
% This definition distinguishes spatial bias from several related concepts. 
% A \emph{spatial error} refers to any incorrect prediction and may occur randomly, whereas spatial bias requires a consistent directional tendency across examples. 
% A \emph{hallucination} describes an output unsupported by the image, while spatial bias characterizes the systematic preference that may contribute to such hallucinations. 
% Similarly, poor spatial reasoning capability indicates limited task performance in general, whereas spatial bias specifically concerns the \emph{structure and direction} of the resulting errors.

% Therefore, our objective is not only to measure whether VLMs make spatial mistakes, but to determine whether they \emph{prefer certain spatial interpretations over others in a systematic manner}.

\textbf{Taxonomy: What spatial bias is observed.}
We categorize spatial bias into six complementary dimensions, as depicted in Fig.~\ref{fig:bias_type}. Specifically, \textit{Spatial Position Bias} denotes systematic preferences for particular absolute or image-relative locations, such as favoring objects in frequently observed image regions; \textit{Spatial Relationship Bias} captures asymmetric reasoning over pairwise relations, including left/right, above/below, and front/behind; \textit{Geometric Structure Bias} reflects preferences for familiar layouts or geometric configurations, such as alignment, symmetry, ordering, enclosure, and relative arrangement; \textit{Depth and Scale Bias} refers to systematic distortions in relative depth, distance, size, or scale estimation, often driven by apparent image size, vertical position, or familiar object scale; \textit{Viewpoint and Orientation Bias} characterizes sensitivity to camera perspective, object orientation, and reference frame, leading to inconsistent spatial judgments under viewpoint or orientation changes; \textit{Spatial Action Bias} arises when biased spatial understanding propagates to navigation, movement, or interaction decisions, causing systematic preferences for particular actions despite scene constraints.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figs/bias_type.pdf}
    \caption{
    \textbf{Taxonomy of spatial bias in VLMs.} Left: Observable manifestations across six spatial reasoning tasks. Right: Four underlying sources of spatial bias.
    }
    \label{fig:bias_type}
    \vspace{-10pt}
\end{figure}

% \begin{itemize}[nosep,leftmargin=*]
%     \item \textbf{Spatial Position Bias} denotes systematic preferences for particular absolute or image-relative locations, such as favoring objects in frequently observed image regions.

%     \item \textbf{Spatial Relationship Bias} captures asymmetric reasoning over pairwise relations, including left/right, above/below, and front/behind.

%     \item \textbf{Geometric Structure Bias} reflects preferences for familiar layouts or geometric configurations, such as alignment, symmetry, ordering, enclosure, and relative arrangement.

%     \item \textbf{Depth and Scale Bias} refers to systematic distortions in relative depth, distance, size, or scale estimation, often driven by apparent image size, vertical position, or familiar object scale.

%     \item \textbf{Viewpoint and Orientation Bias} characterizes sensitivity to camera perspective, object orientation, and reference frame, leading to inconsistent spatial judgments under viewpoint or orientation changes.

%     \item \textbf{Spatial Action Bias} arises when biased spatial understanding propagates to navigation, movement, or interaction decisions, causing systematic preferences for particular actions despite scene constraints.
% \end{itemize}

\textbf{Sources: Why spatial bias occurs.}
We further consider four prior sources that may induce spatial bias, as shown in Fig.~\ref{fig:bias_type}: 
\textit{Cultural Priors} encode learned conventions, such as traffic rules, common layouts, and behavioral norms, which may favor socially typical spatial configurations; 
\textit{Physical Priors} capture geometric and physical regularities, including perspective, support relations, and force constraints, but may become over-generalized beyond the observed evidence;
\textit{Semantic Priors} arise from frequently observed object semantic co-occurrences and spatial bindings, potentially overriding conflicting visual evidence;
\textit{Reference-frame Priors} reflect dependencies on egocentric or allocentric representations and may induce errors when the required coordinate transformation is not correctly performed.

% \begin{itemize}[nosep,leftmargin=*]
%     \item \textbf{Cultural Priors} encode learned conventions, such as traffic rules, common layouts, and behavioral norms, which may favor socially typical spatial configurations.

%     \item \textbf{Physical Priors} capture geometric and physical regularities, including perspective, support relations, and force constraints, but may become over-generalized beyond the observed evidence.

%     \item \textbf{Semantic Priors} arise from frequently observed object semantic co-occurrences and spatial bindings, potentially overriding conflicting visual evidence.

%     \item \textbf{Reference-frame Priors} reflect dependencies on egocentric or allocentric representations and may induce errors when the required coordinate transformation is not correctly performed.
% \end{itemize}

Overall, the taxonomy characterizes \emph{what} forms spatial bias takes, while the source analysis provides complementary hypotheses for \emph{why} such biases emerge.


% \textbf{Taxonomy: What spatial bias is observed.}
% Based on the spatial factors required for visual understanding and embodied interaction, we categorize spatial bias into six complementary dimensions, as illustrated in Fig.~\ref{fig:bias_type}.

% \begin{figure}
%     \centering
%     \includegraphics[width=1\linewidth]{figs/bias_type.pdf}
%     \caption{The phenomenon of spatial bias in VLMs and the categorization of spatial bias classified by the specific manifestations across various spatial reasoning tasks (left) and underlying causes of the spatial bias (right). O refers original and CF denotes counterfactual. 
%     }
%     \label{fig:bias_type}
% \end{figure}

% \begin{itemize}[leftmargin=*]
%     \item \textbf{Spatial Position Bias} refers to a model's systematic preference for particular absolute or image-relative locations.  For example, when otherwise comparable objects are moved among different regions of an image, a VLM may disproportionately predict objects located near the image center, upper region, or other frequently observed positions. Such bias reflects location priors learned from non-uniform spatial distributions in training data.
%     \item \textbf{Spatial Relationship Bias} concerns systematic asymmetries in pairwise spatial reasoning, such as \emph{left/right}, \emph{above/below}, \emph{front/behind}, and \emph{near/far}. A model may, for instance, correctly recognize one directional relation while failing disproportionately on its inverse, even when the corresponding visual evidence is equally salient. This type of bias directly affects relational grounding and compositional spatial reasoning.
%     \item \textbf{Geometric Structure Bias} describes preferences toward particular spatial layouts or geometric arrangements, including alignment, symmetry, ordering, enclosure, and relative configuration. VLMs may favor frequently observed geometric patterns over less common but visually valid alternatives, causing incorrect interpretations when the arrangement deviates from learned structural priors.
%     \item \textbf{Depth and Scale Bias} refers to systematic errors in estimating relative depth, distance, size, or scale. For example, models may over-rely on apparent image size, vertical image position, or familiar object size when determining which object is closer or larger. Such behavior reveals a dependence on monocular or semantic heuristics rather than robust geometric inference.
%     \item \textbf{Viewpoint and Orientation Bias} captures sensitivity to camera perspective, object heading, and reference frame.  A spatial relation that is correctly interpreted from one viewpoint may become systematically misclassified after viewpoint rotation or orientation reversal. This bias is particularly important for transformations between egocentric and allocentric representations, where spatial relations must be recomputed rather than recalled from image-level patterns.
%     \item \textbf{Spatial Action Bias} arises when spatial perception errors propagate into predictions of movement, navigation, or interaction. Given comparable scenes, a VLM may systematically favor particular motion directions, turning behaviors, or navigation choices due to learned behavioral priors rather than the actual spatial constraints of the scene. This category connects spatial perception to embodied decision making and therefore represents a higher-level consequence of spatial bias.
% \end{itemize}


% \textbf{Sources: Why spatial bias occurs.}
% Beyond the observable bias categories above, we further consider four representative sources that may induce spatial bias. 
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Cultural Priors (Cultural and Behavioral Norms)} encode regularities such as traffic rules and conventional facility layouts, which may encourage models to prefer socially common spatial arrangements. 
%     \item \textbf{Physical Priors (Physical and Geometric Principles)}, including perspective projection, support relations, and force equilibrium, provide strong real-world regularities but may also become over-generalized priors. 
%     \item \textbf{Semantic Priors (Semantic Co-occurrence)} captures frequently observed spatial bindings, such as pedestrians near crossings or screens positioned above keyboards, which can override conflicting visual evidence. 
%     \item \textbf{Reference-frame Priors (Egocentric--allocentric Transformation)} introduces reference-frame dependence, making spatial judgments vulnerable when models fail to correctly transform between observer-centered and world-centered coordinates.
% \end{itemize}

% % These sources are not mutually exclusive. 
% % A single spatial prediction may simultaneously reflect semantic, geometric, behavioral, and viewpoint priors. 
% Our taxonomy therefore characterizes \emph{what} spatial bias manifests, while the above sources help explain \emph{why} such bias may emerge.

\textbf{Notations.}
Let $N$ denote the number of original images captured from the drone's embodied view, with $\mathbb{I}^{O}=\{I_i^{O}\}_{i=1}^{N}$.
For each original image, a controlled spatial transformation $\mathcal{T}_i$ modifies the target spatial factor while preserving task-irrelevant semantic content, yielding the counterfactual image $I_i^{CF}=\mathcal{T}_i(I_i^{O})$.
We denote the counterfactual image set as $\mathbb{I}^{CF}=\{I_i^{CF}\}_{i=1}^{N}$ and the complete image set as $\mathbb{I}=\mathbb{I}^{O}\cup\mathbb{I}^{CF}$.
%
Let $q_i\in\mathbb{Q}$ denote the spatial query associated with the $i$th image pair.
The original and counterfactual VQ sets are $\mathcal{V}^{O}=\{(I_i^{O},q_i)\}_{i=1}^{N}$ and $\mathcal{V}^{CF}=\{(I_i^{CF},q_i)\}_{i=1}^{N}$, with $\mathcal{V}=\mathcal{V}^{O}\cup\mathcal{V}^{CF}$.
Given an image--question pair $(I,q)\in\mathcal{V}$, a VLM $\mathcal{M}$ predicts $\hat y=\mathcal{M}(I,q)$.
Accordingly, $\hat y_i^{O}=\mathcal{M}(I_i^{O},q_i)$ and $\hat y_i^{CF}=\mathcal{M}(I_i^{CF},q_i)$ denote the predictions for the original and counterfactual inputs, with corresponding ground-truth answers $y_i^{O}$ and $y_i^{CF}$.

% \textbf{Notations.}
% Let $N$ be the total amount number of original images obtained from the UAV's embodied view, and $\mathbb{I}^O=\{I^O_i\}_{0<i\leq N}$ be the set of original images. 
% %
% Let $\mathcal{T}$ denote a controlled spatial transformation that modifies a target spatial factor while preserving task-irrelevant semantic content of the original images, producing a set of counterfactual images $\mathbb{I}^{CF}=\{I^{CF}_i\}_{0<i\leq N}=\{\mathcal{T}_i(I^O_i)\}_{0<i\leq N}$.
% The entire image set is $\mathbb{I}=\mathbb{I}^O \cup \mathbb{I}^{CF}$.
% %
% Let $\hat y=\mathcal{M}(I,q)$ denote the output answer by a VLM $\mathcal{M}$ for an image-question pair $(I,q)\in\mathcal{V}$, where $I\in\mathbb{I}$ is the input image, $q\in\mathbb{Q}$ is a spatial query, and $\mathcal{V}=\mathcal{V}^O\cup\mathcal{V}^{CF}$ is the set of all visual-question (VQ) pairs. 
% We denote the model's predicted answer for the $i$th original and counterfactual VQ pair as $\hat y^O_i=\mathcal{M}(I^O_i,q_i)$ and $\hat y^{CF}_i=\mathcal{M}(I^{CF}_i,q_i)$, respectively. 
% Correspondingly, the ground-truth answer of the $i$th original and counterfactual input pair is defined as $y^O_i$ and $y^{CF}_i$, respectively. 
 
% \textbf{Benchmark.}



==> sections/app_data_filter.tex <==
{\color{black}
\subsubsection{Effects of Data Filtering: Filtered vs. Unfiltered}
\label{app:filtering}

Our data curation aims to focus the benchmark on prior reliance rather than general recognition failures. Consistent with our diagnostic framework, bias metrics are computed on model-specific eligible samples where the original image is answered correctly. During curation, 43 pairs were excluded because all three curation models incorrectly answered the original image but correctly answered its counterfactual, suggesting that these edits may not effectively challenge the intended spatial priors. Such outcomes are not inherently invalid and remain present in the curated benchmark. To verify the robustness of our findings, we conduct an additional sensitivity analysis by including these 43 pairs and recomputing all metrics for 17 models on the complete 1,297-pair pool under the original evaluation settings.

As shown in Tab.~\ref{tab:app_filtering}, the differences between the filtered and unfiltered results are minor. Across all models, BR changes by $-0.54$ to $+0.08$ pp, with a mean change of $-0.23$ pp. The changes in $\mathrm{Acc}^{O}$ and $\mathrm{Acc}^{CF}$ range from $-1.85$ to $-0.05$ pp and $+0.05$ to $+1.86$ pp, respectively. Importantly, the BR rankings remain unchanged (Spearman's $\rho=1.000$, Kendall's $\tau=1.000$), as do the rankings for pAcc and mAcc. Other bias-related metrics, including PRR, LBR, and CER, also exhibit limited variation.
%
Fig.~\ref{fig:four_way} further compares the four original--counterfactual correctness outcomes before and after filtering. Original-incorrect/counterfactual-correct cases remain present in both datasets, and including the 43 excluded pairs produces only minor changes in the overall outcome distribution. These results demonstrate that the main findings and cross-model BR comparisons are robust to the data filtering procedure.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figs/four_way_composition.pdf}
    \vspace{-8pt}
    \caption{\textcolor{black}{\textbf{Four-way composition of the O/CF outcomes before and after the pre-filter.} Solid bars: the 1254 filtered pairs; hatched: the 1297-pair pool with the 43 excluded pairs re-run. Colours give the four correctness combinations (green: both correct; pink: original correct only; orange: counterfactual correct only; black: both wrong), and the numbers inside the bars are percentages of the pool. Middle strip: $\mathrm{BR}$ per model (filled dot: filtered; open square: unfiltered); lower strip: the change of each cell in points. 
    % The four changes sum to zero by construction, and bars stop short of 100\% where a pair has no usable answer on one side.
    }}
    \label{fig:four_way}
    \vspace{-10pt}
\end{figure}

\input{tables/appendix_filtering}

}


==> tables/full_background.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Comprehensive evaluation results of background information ablation study.}
A0 denotes the baseline evaluation on original images.
B1 ($\sigma \in \{4, 8, 12, 15\}$) denotes background perturbation with varying Gaussian blur strengths applied to non-target regions.
B2 ($\sigma=8$) denotes full-image background perturbation.
B3 denotes visual prompting with bounding box annotation.
Accuracy metrics ($Acc_{O}$, $Acc_{CF}$, $pAcc$, $mAcc$) are reported alongside robust evaluation indicators ($PRR$, $LBR$, $BR$, $CER$, $NBER$, $LPD$, and $TOR$).
Accuracy denominators are fixed at 1254 pairs.}
\label{tab:background_ablation_full}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccccccccccc}
\toprule
\textbf{Model} & \textbf{Config.} & \textbf{N} & 
$\mathbf{Acc_{O}}\uparrow$ & $\mathbf{Acc_{CF}}\uparrow$ & $\mathbf{pAcc}\uparrow$ & $\mathbf{mAcc}\uparrow$ & 
$\mathbf{PRR}\downarrow$ & $\mathbf{LBR}\downarrow$ & $\mathbf{BR}\downarrow$ & $\mathbf{CER}\downarrow$ & 
$\mathbf{NBER}\downarrow$ & $\mathbf{LPD}\downarrow$ & $\mathbf{TOR}\downarrow$ \\
\midrule

\multirow{7}{*}{Gemini 3.8 Flash}
& A0 & 939 & 0.7560 & 0.4896 & 0.3724 & 0.6228 & 0.4483 & 0.3568 & 0.4505 & 0.5091 & 0.0586 & 0.6705 & 0.4646 \\
& B1 $\sigma=4$ & 948 & 0.7584 & 0.5183 & 0.4099 & 0.6384 & 0.4082 & 0.3186 & 0.4114 & 0.4599 & 0.0485 & 0.6737 & 0.4114 \\
& B1 $\sigma=8$ & 967 & 0.7719 & 0.5247 & 0.4195 & 0.6483 & 0.4105 & 0.3299 & 0.4178 & 0.4571 & 0.0393 & 0.6794 & 0.4270 \\
& B1 $\sigma=12$ & 955 & 0.7624 & 0.5064 & 0.3995 & 0.6344 & 0.4209 & 0.3309 & 0.4304 & 0.4764 & 0.0461 & 0.6743 & 0.4282 \\
& B1 $\sigma=15$ & 948 & 0.7592 & 0.5064 & 0.4027 & 0.6328 & 0.4146 & 0.3397 & 0.4219 & 0.4684 & 0.0464 & 0.6919 & 0.4334 \\
& B2 $\sigma=8$ & 904 & 0.7257 & 0.3804 & 0.2648 & 0.5530 & 0.5830 & 0.4712 & 0.5885 & 0.6372 & 0.0487 & 0.7052 & 0.5900 \\
& B3 & 975 & 0.7799 & 0.5415 & 0.4234 & 0.6607 & 0.4103 & 0.3262 & 0.4174 & 0.4564 & 0.0390 & 0.6687 & 0.4234 \\

\midrule

\multirow{7}{*}{GPT-5.6 terra}
& A0 & 945 & 0.7560 & 0.4043 & 0.2951 & 0.5801 & 0.5439 & 0.4794 & 0.5661 & 0.6106 & 0.0444 & 0.7159 & 0.5815 \\
& B1 $\sigma=4$ & 926 & 0.7416 & 0.4402 & 0.2990 & 0.5909 & 0.5421 & 0.4806 & 0.5551 & 0.5961 & 0.0410 & 0.7266 & 0.5640 \\
& B1 $\sigma=8$ & 949 & 0.7592 & 0.4330 & 0.3006 & 0.5961 & 0.5627 & 0.5037 & 0.5753 & 0.6038 & 0.0285 & 0.7421 & 0.5894 \\
& B1 $\sigma=12$ & 945 & 0.7560 & 0.4330 & 0.2974 & 0.5945 & 0.5619 & 0.5132 & 0.5757 & 0.6074 & 0.0317 & 0.7474 & 0.5980 \\
& B1 $\sigma=15$ & 914 & 0.7432 & 0.4482 & 0.3134 & 0.5957 & 0.5328 & 0.4836 & 0.5460 & 0.5744 & 0.0284 & 0.7301 & 0.5595 \\
& B2 $\sigma=8$ & 823 & 0.6587 & 0.3038 & 0.1427 & 0.4813 & 0.7351 & 0.6476 & 0.7485 & 0.7849 & 0.0365 & 0.7900 & 0.7372 \\
& B3 & 899 & 0.7177 & 0.5494 & 0.3724 & 0.6336 & 0.4271 & 0.3482 & 0.4372 & 0.4816 & 0.0445 & 0.6407 & 0.4372 \\

\midrule

\multirow{7}{*}{Qwen3-VL-32B}
& A0  & 842 & 0.6730 & 0.3469 & 0.1962 & 0.5100 & 0.6366 & 0.5499 & 0.6651 & 0.7090 & 0.0439 & 0.7209 & 0.6182 \\
& B1 $\sigma=4$ & 852 & 0.6810 & 0.3836 & 0.2376 & 0.5323 & 0.5904 & 0.5082 & 0.6103 & 0.6526 & 0.0423 & 0.6995 & 0.5773 \\
& B1 $\sigma=8$ & 842 & 0.6730 & 0.3780 & 0.2392 & 0.5255 & 0.5724 & 0.5131 & 0.6069 & 0.6461 & 0.0392 & 0.6948 & 0.5822 \\
& B1 $\sigma=12$ & 822 & 0.6571 & 0.3820 & 0.2368 & 0.5195 & 0.5657 & 0.4951 & 0.5912 & 0.6411 & 0.0499 & 0.6971 & 0.5645 \\
& B1 $\sigma=15$ & 822 & 0.6571 & 0.3812 & 0.2344 & 0.5191 & 0.5693 & 0.4988 & 0.5985 & 0.6448 & 0.0462 & 0.6861 & 0.5702 \\
& B2  $\sigma=8$ & 765 & 0.6116 & 0.2305 & 0.0917 & 0.4211 & 0.7817 & 0.6797 & 0.8118 & 0.8523 & 0.0405 & 0.7516 & 0.7569 \\
& B3  & 877 & 0.7010 & 0.4234 & 0.2671 & 0.5622 & 0.5405 & 0.4778 & 0.5781 & 0.6203 & 0.0422 & 0.6796 & 0.5420 \\

\midrule

\multirow{7}{*}{Qwen3-VL-8B}
& A0  & 832 & 0.6651 & 0.2831 & 0.1539 & 0.4741 & 0.7212 & 0.6022 & 0.7284 & 0.7704 & 0.0421 & 0.7392 & 0.6779 \\
& B1 $\sigma=4$ & 826 & 0.6603 & 0.3134 & 0.1914 & 0.4868 & 0.6550 & 0.5787 & 0.6659 & 0.7119 & 0.0460 & 0.7421 & 0.6442 \\
& B1 $\sigma=8$ & 811 & 0.6483 & 0.3126 & 0.1866 & 0.4805 & 0.6510 & 0.5746 & 0.6658 & 0.7139 & 0.0481 & 0.7337 & 0.6445 \\
& B1 $\sigma=12$ & 809 & 0.6467 & 0.3174 & 0.1930 & 0.4821 & 0.6391 & 0.5711 & 0.6539 & 0.7033 & 0.0494 & 0.7231 & 0.6426 \\
& B1 $\sigma=15$ & 789 & 0.6308 & 0.3214 & 0.1930 & 0.4761 & 0.6324 & 0.5678 & 0.6477 & 0.6958 & 0.0482 & 0.7237 & 0.6391 \\
& B2  $\sigma=8$ & 672 & 0.5367 & 0.1938 & 0.0758 & 0.3652 & 0.7932 & 0.6622 & 0.8095 & 0.8601 & 0.0506 & 0.7679 & 0.7248 \\
& B3  & 831 & 0.6643 & 0.3517 & 0.2193 & 0.5080 & 0.6185 & 0.5343 & 0.6258 & 0.6715 & 0.0457 & 0.7256 & 0.6008 \\

\midrule

\multirow{7}{*}{Qwen3-VL-2B}
& A0  & 621 & 0.4952 & 0.3333 & 0.1021 & 0.4143 & 0.7198 & 0.5282 & 0.7488 & 0.7939 & 0.0451 & 0.6087 & 0.6586 \\
& B1 $\sigma=4$ & 611 & 0.4872 & 0.3604 & 0.1340 & 0.4238 & 0.6432 & 0.5188 & 0.6727 & 0.7250 & 0.0524 & 0.6187 & 0.6290 \\
& B1 $\sigma=8$ & 610 & 0.4864 & 0.3525 & 0.1292 & 0.4195 & 0.6541 & 0.5230 & 0.6852 & 0.7344 & 0.0492 & 0.6246 & 0.6280 \\
& B1 $\sigma=12$ & 611 & 0.4872 & 0.3413 & 0.1148 & 0.4143 & 0.6743 & 0.5450 & 0.7152 & 0.7643 & 0.0491 & 0.6252 & 0.6555 \\
& B1 $\sigma=15$ & 617 & 0.4928 & 0.3429 & 0.1260 & 0.4179 & 0.6499 & 0.5267 & 0.6937 & 0.7439 & 0.0502 & 0.6191 & 0.6335 \\
& B2  $\sigma=8$ & 521 & 0.4155 & 0.2831 & 0.0383 & 0.3493 & 0.8311 & 0.6372 & 0.8618 & 0.9079 & 0.0461 & 0.7006 & 0.7461 \\
& B3  & 608 & 0.4848 & 0.3828 & 0.1380 & 0.4338 & 0.6316 & 0.5066 & 0.6694 & 0.7155 & 0.0461 & 0.6266 & 0.6123 \\

\midrule

\multirow{7}{*}{\shortstack[l]{SpatioLM-\\InternVL3.5}}
& A0  & 639 & 0.5112 & 0.2352 & 0.0789 & 0.3732 & 0.7543 & 0.6228 & 0.7934 & 0.8482 & 0.0548 & 0.6823 & 0.7082 \\
& B1 $\sigma=4$ & 657 & 0.5255 & 0.2344 & 0.0821 & 0.3800 & 0.7336 & 0.6012 & 0.7656 & 0.8463 & 0.0807 & 0.6865 & 0.6741 \\
& B1 $\sigma=8$ & 645 & 0.5159 & 0.2376 & 0.0797 & 0.3768 & 0.7333 & 0.5984 & 0.7659 & 0.8481 & 0.0822 & 0.6899 & 0.6784 \\
& B1 $\sigma=12$ & 647 & 0.5175 & 0.2504 & 0.0965 & 0.3840 & 0.7048 & 0.5842 & 0.7326 & 0.8161 & 0.0835 & 0.6940 & 0.6632 \\
& B1 $\sigma=15$ & 641 & 0.5128 & 0.2496 & 0.0957 & 0.3812 & 0.6942 & 0.5881 & 0.7270 & 0.8159 & 0.0889 & 0.6989 & 0.6696 \\
& B2  $\sigma=8$ & 602 & 0.4817 & 0.1938 & 0.0415 & 0.3377 & 0.8322 & 0.6694 & 0.8488 & 0.9169 & 0.0681 & 0.7359 & 0.7463 \\
& B3  & 606 & 0.4841 & 0.2384 & 0.0837 & 0.3612 & 0.7211 & 0.6073 & 0.7525 & 0.8284 & 0.0759 & 0.6997 & 0.6853 \\

\midrule

\multirow{7}{*}{InternVL3.5-8B}
& A0  & 654 & 0.5231 & 0.2839 & 0.0813 & 0.4035 & 0.7813 & 0.6391 & 0.8180 & 0.8471 & 0.0291 & 0.7003 & 0.7013 \\
& B1 $\sigma=4$ & 696 & 0.5566 & 0.3126 & 0.1188 & 0.4346 & 0.7126 & 0.5891 & 0.7572 & 0.7888 & 0.0316 & 0.6580 & 0.6571 \\
& B1 $\sigma=8$ & 684 & 0.5470 & 0.3174 & 0.1228 & 0.4322 & 0.7032 & 0.5760 & 0.7354 & 0.7778 & 0.0424 & 0.6696 & 0.6417 \\
& B1 $\sigma=12$ & 680 & 0.5439 & 0.3222 & 0.1252 & 0.4330 & 0.6941 & 0.5735 & 0.7309 & 0.7721 & 0.0412 & 0.6647 & 0.6404 \\
& B1 $\sigma=15$ & 682 & 0.5455 & 0.3262 & 0.1308 & 0.4358 & 0.6848 & 0.5660 & 0.7214 & 0.7625 & 0.0411 & 0.6628 & 0.6307 \\
& B2  $\sigma=8$ & 597 & 0.4777 & 0.2344 & 0.0383 & 0.3561 & 0.8693 & 0.7052 & 0.8878 & 0.9229 & 0.0352 & 0.7471 & 0.7711 \\
& B3  & 629 & 0.5032 & 0.3285 & 0.1156 & 0.4159 & 0.6932 & 0.6184 & 0.7329 & 0.7727 & 0.0397 & 0.6948 & 0.6825 \\

\midrule

\multirow{7}{*}{SpatialRGPT-8B}
& A0  & 591 & 0.4721 & 0.2480 & 0.0399 & 0.3600 & 0.8528 & 0.7157 & 0.8917 & 0.9171 & 0.0254 & 0.7327 & 0.7790 \\
& B1 $\sigma=4$ & 587 & 0.4689 & 0.2648 & 0.0558 & 0.3668 & 0.8007 & 0.7070 & 0.8450 & 0.8825 & 0.0375 & 0.7411 & 0.7643 \\
& B1 $\sigma=8$ & 573 & 0.4577 & 0.2616 & 0.0502 & 0.3596 & 0.8080 & 0.7225 & 0.8447 & 0.8918 & 0.0471 & 0.7574 & 0.7841 \\
& B1 $\sigma=12$ & 558 & 0.4458 & 0.2600 & 0.0502 & 0.3529 & 0.7975 & 0.7419 & 0.8441 & 0.8889 & 0.0448 & 0.7742 & 0.8008 \\
& B1 $\sigma=15$ & 551 & 0.4402 & 0.2560 & 0.0494 & 0.3481 & 0.7967 & 0.7441 & 0.8475 & 0.8893 & 0.0417 & 0.7695 & 0.8039 \\
& B2  $\sigma=8$ & 541 & 0.4322 & 0.2121 & 0.0128 & 0.3222 & 0.9409 & 0.7930 & 0.9593 & 0.9723 & 0.0129 & 0.7967 & 0.8428 \\
& B3  & 583 & 0.4657 & 0.2751 & 0.0566 & 0.3704 & 0.7959 & 0.7033 & 0.8439 & 0.8799 & 0.0360 & 0.7393 & 0.7649 \\

\bottomrule
\end{tabular}}
\end{table*}

==> tables/input.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Effects of different input configurations.}
A0: \emph{independent single-turn multi-dialogue}, where the O and CF samples are evaluated independently;
A1 and A2: \emph{sequential multi-turn single-dialogue} evaluation, with O$\rightarrow$CF and CF$\rightarrow$O input orders, respectively;
A3: \emph{joint single-turn single-dialogue} evaluation, where O and CF are provided simultaneously in a single turn.
Values in parentheses indicate percentage-point (pp) changes relative to A0 for the same model, with \textcolor{red}{red} and \textcolor{green!60!black}{green} denoting increases and decreases, respectively.}
\label{tab:configuration_delta}
\resizebox{\textwidth}{!}{
\begin{tabular}{llccccccc}
\toprule
\textbf{Model} & \textbf{Config.} &
$\mathbf{Acc^{O}}\uparrow$ &
$\mathbf{Acc^{CF}}\uparrow$ &
$\mathbf{pAcc}\uparrow$ &
$\mathbf{PRR}\downarrow$ &
$\mathbf{LBR}\downarrow$ &
$\mathbf{BR}\downarrow$ &
$\mathbf{CER}\downarrow$ \\
\midrule

\multirow{4}{*}{Qwen3-VL-8B}
& A0
& 0.668 & 0.300 & 0.160
& 0.707 & 0.611 & 0.722 & 0.761 \\

& A1
& 0.665 {\scriptsize \textcolor{green!60!black}{($\mathbf{-0.3}$)}}
& 0.193 {\scriptsize \textcolor{green!60!black}{($\mathbf{-10.7}$)}}
& 0.059 {\scriptsize \textcolor{green!60!black}{($\mathbf{-10.1}$)}}
& 0.900 {\scriptsize \textcolor{red}{($\mathbf{+19.3}$)}}
& 0.686 {\scriptsize \textcolor{red}{($\mathbf{+7.6}$)}}
& 0.903 {\scriptsize \textcolor{red}{($\mathbf{+18.1}$)}}
& 0.914 {\scriptsize \textcolor{red}{($\mathbf{+15.2}$)}} \\

& A2
& 0.565 {\scriptsize \textcolor{green!60!black}{($\mathbf{-10.3}$)}}
& 0.283 {\scriptsize \textcolor{green!60!black}{($\mathbf{-1.7}$)}}
& 0.051 {\scriptsize \textcolor{green!60!black}{($\mathbf{-10.9}$)}}
& 0.895 {\scriptsize \textcolor{red}{($\mathbf{+18.8}$)}}
& 0.734 {\scriptsize \textcolor{red}{($\mathbf{+12.4}$)}}
& 0.901 {\scriptsize \textcolor{red}{($\mathbf{+17.9}$)}}
& 0.912 {\scriptsize \textcolor{red}{($\mathbf{+15.1}$)}} \\

& A3
& 0.549 {\scriptsize \textcolor{green!60!black}{($\mathbf{-12.0}$)}}
& 0.245 {\scriptsize \textcolor{green!60!black}{($\mathbf{-5.5}$)}}
& 0.054 {\scriptsize \textcolor{green!60!black}{($\mathbf{-10.6}$)}}
& 0.882 {\scriptsize \textcolor{red}{($\mathbf{+17.5}$)}}
& 0.693 {\scriptsize \textcolor{red}{($\mathbf{+8.2}$)}}
& 0.884 {\scriptsize \textcolor{red}{($\mathbf{+16.2}$)}}
& 0.903 {\scriptsize \textcolor{red}{($\mathbf{+14.1}$)}} \\

\midrule

\multirow{4}{*}{SpatioLM}
& A0
& 0.511 & 0.235 & 0.079
& 0.754 & 0.623 & 0.793 & 0.848 \\

& A1
& 0.511 
& 0.160 {\scriptsize \textcolor{green!60!black}{($\mathbf{-7.5}$)}}
& 0.010 {\scriptsize \textcolor{green!60!black}{($\mathbf{-6.9}$)}}
& 0.975 {\scriptsize \textcolor{red}{($\mathbf{+22.1}$)}}
& 0.676 {\scriptsize \textcolor{red}{($\mathbf{+5.3}$)}}
& 0.980 {\scriptsize \textcolor{red}{($\mathbf{+18.6}$)}}
& 0.983 {\scriptsize \textcolor{red}{($\mathbf{+13.5}$)}} \\

& A2
& 0.422 {\scriptsize \textcolor{green!60!black}{($\mathbf{-8.9}$)}}
& 0.235 {\scriptsize ($+0.0$)}
& 0.013 {\scriptsize \textcolor{green!60!black}{($\mathbf{-6.6}$)}}
& 0.964 {\scriptsize \textcolor{red}{($\mathbf{+21.0}$)}}
& 0.742 {\scriptsize \textcolor{red}{($\mathbf{+11.9}$)}}
& 0.968 {\scriptsize \textcolor{red}{($\mathbf{+17.4}$)}}
& 0.973 {\scriptsize \textcolor{red}{($\mathbf{+12.5}$)}} \\

& A3
& 0.443 {\scriptsize \textcolor{green!60!black}{($\mathbf{-6.8}$)}}
& 0.164 {\scriptsize \textcolor{green!60!black}{($\mathbf{-7.1}$)}}
& 0.002 {\scriptsize \textcolor{green!60!black}{($\mathbf{-7.7}$)}}
& 1.000 {\scriptsize \textcolor{red}{($\mathbf{+24.6}$)}}
& 0.681 {\scriptsize \textcolor{red}{($\mathbf{+5.8}$)}}
& 1.000 {\scriptsize \textcolor{red}{($\mathbf{+20.7}$)}}
& 1.000 {\scriptsize \textcolor{red}{($\mathbf{+15.2}$)}} \\

\midrule

\multirow{4}{*}{GPT-5.6 Terra}
& A0
& 0.756 & 0.404 & 0.295
& 0.544 & 0.479 & 0.566 & 0.611 \\

& A1
& 0.709 {\scriptsize \textcolor{green!60!black}{($\mathbf{-4.7}$)}}
& 0.542 {\scriptsize \textcolor{red}{($\mathbf{+13.8}$)}}
& 0.372 {\scriptsize \textcolor{red}{($\mathbf{+7.7}$)}}
& 0.412 {\scriptsize \textcolor{green!60!black}{($\mathbf{-13.2}$)}}
& 0.338 {\scriptsize \textcolor{green!60!black}{($\mathbf{-14.1}$)}}
& 0.422 {\scriptsize \textcolor{green!60!black}{($\mathbf{-14.5}$)}}
& 0.476 {\scriptsize \textcolor{green!60!black}{($\mathbf{-13.5}$)}} \\

& A2
& 0.708 {\scriptsize \textcolor{green!60!black}{($\mathbf{-4.8}$)}}
& 0.420 {\scriptsize \textcolor{red}{($\mathbf{+1.6}$)}}
& 0.297 {\scriptsize \textcolor{red}{($\mathbf{+0.2}$)}}
& 0.490 {\scriptsize \textcolor{green!60!black}{($\mathbf{-5.4}$)}}
& 0.453 {\scriptsize \textcolor{green!60!black}{($\mathbf{-2.7}$)}}
& 0.520 {\scriptsize \textcolor{green!60!black}{($\mathbf{-4.6}$)}}
& 0.580 {\scriptsize \textcolor{green!60!black}{($\mathbf{-3.1}$)}} \\

& A3
& 0.703 {\scriptsize \textcolor{green!60!black}{($\mathbf{-5.3}$)}}
& 0.569 {\scriptsize \textcolor{red}{($\mathbf{+16.4}$)}}
& 0.360 {\scriptsize \textcolor{red}{($\mathbf{+6.5}$)}}
& 0.429 {\scriptsize \textcolor{green!60!black}{($\mathbf{-11.5}$)}}
& 0.353 {\scriptsize \textcolor{green!60!black}{($\mathbf{-12.7}$)}}
& 0.444 {\scriptsize \textcolor{green!60!black}{($\mathbf{-12.2}$)}}
& 0.489 {\scriptsize \textcolor{green!60!black}{($\mathbf{-12.1}$)}} \\

\bottomrule
\end{tabular}}
\end{table*}


==> tables/metrics.tex <==

\begin{table*}[htbp]
\centering
\caption{Definitions and calculations of evaluation metrics for each research question.}
\label{tab:metrics}

\renewcommand{\arraystretch}{1.5} % 拉高行距，给分式留出呼吸空间
\setlength{\tabcolsep}{4pt}      % 微调列间距

% 使用 \scalebox{0.85} 整体缩放表格，确保不超出页面边界
\scalebox{0.77}{%
\begin{tabular}{
    >{\raggedright\arraybackslash}p{1.5cm} % Purpose (第1列)
    >{\raggedright\arraybackslash}p{2.5cm} % Metric (第2列)
    >{\centering\arraybackslash}p{7.4cm}   % Formula (第3列：分配 7.5cm 保证公式不折行)
    >{\raggedright\arraybackslash}p{4.5cm} % Interpretation (第4列)
    >{\centering\arraybackslash}p{1.0cm}   % RQ (第5列)
}
\toprule
\textbf{Purpose} & \textbf{Metric} & \textbf{Formula} & \textbf{Interpretation} & \textbf{RQ} \\
\midrule

% Accuracy Performance Section
\multirow{4}{*}{\shortstack[l]{Accuracy\\Diagnosis}} 
{ \color{blue}
 & O Accuracy       & $Acc^O = \frac{1}{|\mathcal{V}|} \sum_{(I_i, q_i) \in \mathcal{V}} \mathds{1}(\hat{y}_i^O = y_i^O)$ & Accuracy on O data & RQ1 \\
 & CF Accuracy             & $Acc^{CF} = \frac{1}{|\mathcal{V}|} \sum_{(I_i, q_i) \in \mathcal{V}} \mathds{1}(\hat{y}_i^{CF} = y_i^{CF})$ & Accuracy on CF data & RQ1 \\
 & Pair Accuracy           & $pAcc = \frac{1}{N}\sum_{(I_i, q_i) \in \mathcal{V}} \mathds{1}(\hat{y}_i^O = y_i^O \land \hat{y}_i^{CF} = y_i^{CF})$ & Pairwise accuracy consistency between O and CF pairs & RQ1 \\
 % & Mean Accuracy           & $mAcc = \frac{1}{|\mathcal{V}|}{\sum_{(I_i, q_i) \in \mathcal{V}} \mathds{1}(\hat{y}_i^O = y_i^O \lor \hat{y}_i^{CF} = y_i^{CF})}$ & Average accuracy across all O and CF data & RQ1 \\
 & Mean Accuracy           & $mAcc = \frac{1}{2}(Acc^O+Acc^{CF})$ & Average accuracy across all O and CF data & RQ1 \\
}
\midrule

% Failure Diagnosis Section
\multirow{2}{*}{\shortstack[l]{Failure\\Diagnosis}} 
 & CF Error Rate           & $CER = \frac{1}{|\mathcal{E}|}{\sum_{i \in \mathcal{E}} \mathds{1}(\hat{y}_i^{CF} \neq y_i^{CF})}$ & Failure rate from counterfactual perturbation & RQ2 \\
 & Non-bias CF Error Rate       & $NBER = CER - BR$ & Failure rate unrelated to spatial bias & RQ2 \\
\midrule

% Bias Diagnosis Section
\multirow{5}{*}{\shortstack[l]{Bias\\Diagnosis}} 
 & Prior Retention Rate      & $PRR = \frac{1}{|\mathcal{E}|}{\sum_{i \in \mathcal{E}} \mathds{1}(\hat{y}_i^{CF} = y_i^O)}$ & Rate of CF prediction clinging to original ground truth & RQ3 \\
 & Bias Rate                 & $BR = \frac{1}{|\mathcal{E}|} \sum_{i \in \mathcal{E}}\mathds{1}(i \in \mathcal{B})$ & Proportion of CF spatial errors attributed to spatial bias & RQ3 \\
 & Language-prior Dependency 
 & $LPD=\frac{1}{|\mathcal{E}|}{\sum_{i\in\mathcal{E}}\mathds{1}(\hat y^{T}_i=y^O_i)}$ 
 & Model dependency on pure language priors & RQ4 \\
 & Text Override Rate 
 & $TOR=\frac{1}{|\mathcal{C}|}{\sum_{i\in\mathcal{C}}\mathds{1}(\hat y^{CF}_i=\hat y^T)}$ 
 & Rate of text overriding visual evidence & RQ5 \\
 & Language-prior Bias Rate  
 & $LBR=\frac{1}{|\mathcal{E}|}{\sum_{i\in\mathcal{E}}\mathds{1}(y^{CF}_i=\hat y^{T}_i \land\hat y^T_i\neq y^{CF}_i)}$
 & Overall spatial bias rate from language priors & RQ6 \\
\bottomrule
\end{tabular}%
}
\vspace{-10pt}
\end{table*}
